Summarizing Community-based Question-Answer Pairs

Community-based Question Answering (CQA), which allows users to acquire their desired information, has increasingly become an essential component of online services in various domains such as E-commerce, travel, and dining. However, an overwhelming number of CQA pairs makes it difficult for users without particular intent to find useful information spread over CQA pairs. To help users quickly digest the key information, we propose the novel CQA summarization task that aims to create a concise summary from CQA pairs. To this end, we first design a multi-stage data annotation process and create a benchmark dataset, CoQASUM, based on the Amazon QA corpus. We then compare a collection of extractive and abstractive summarization methods and establish a strong baseline approach DedupLED for the CQA summarization task. Our experiment further confirms two key challenges, sentence-type transfer and deduplication removal, towards the CQA summarization task. Our data and code are publicly available.

==> EMNLP-2022 CoQASum/sections/abstract.tex <==
%E-service platforms have been widely used in our daily life. People browse the websites and tend to post questions naturally. Some people would answers those questions based on their understanding, experiences or even external knowledges. Those questions and answers contain rich information about the discussed topic that is called community questions answering (CQA). Thanks for the rich CQA, people can easily obtain information about the things they are looking for. Amazon.com is one of the most popular E-service platforms that huge amount of customers searching and buying product everyday. Due to the rich information from questions and answers, customers may know more about the product that they are interesting in. However, sometimes CQA is too overwhelming for the customer when they are just browsing and not sure what specific questions to ask. Furthermore, many Q\&As are repetitive and the responsive answers are not useful that could confuse the customers. To solve below problem, we propose QA summarization (cool name maybe), a novel QA summarization task. Our goal is not only remove the repetitive Q\&As, but also summarize multiple Q\&As into a declarative format that can provide customers the key or more concrete information of the product. We introduce a new dataset based on the well-known Amazon dataset. Our dataset consists of \todo{put stats}. We do two steps annotation to collect the summary in a better quality. We then established several strong baseline models across three common methods used in existing summarization task, extractive, abstractive and extractive-abstractive. To our best knowledge, we are the first to propose this Q\&A summarization task. We evaluate the experimental results on both autometric and human perspective. We compared numerous models for Q\&A summarization, doing different specific analysis and demonstratd the challenging nature of this new task.

%\hl{E-commerce platforms have been widely used in our daily life for a variety of tasks, such as online shopping, job searching and service booking. An increasingly important component in such e-commerce platforms is the Community Question Answering (CQA) service, which allows users to acquire their desired information. However, the large volume of QAs could easily overwhelm users, especially when they don't have a particular question to ask, but still want to know the key information mentioned by the others. To help users quickly digest information in QAs, we propose a novel \task\ task that targets at producing a concise and declarative summary of the key information in the QAs. Towards this goal, we first design a non-trivial data annotation process and introduce a benchmark dataset, \corpus, based on the Amazon QA corpus. We then compare a collection of extractive and abstractive models for the task. Through our experiment, we established a strong baseline model and demonstrated the challenging nature of the \task\ task. Our data and code are avaialble at \codeurl. }


Community-based Question Answering (CQA), which allows users to acquire their desired information, has increasingly become an essential component of online services in various domains such as E-commerce, travel, and dining. However, an overwhelming number of CQA pairs makes it difficult for users without particular intent to find useful information spread over CQA pairs. To help users quickly digest the key information, we propose the novel \task\ task that aims to create a concise summary from CQA pairs. To this end, we first design a multi-stage data annotation process and create a benchmark dataset, \corpus, based on the Amazon QA corpus. We then compare a collection of extractive and abstractive summarization methods and establish a strong baseline approach DedupLED for the \task\ task. Our experiment further confirms two key challenges, sentence-type transfer and deduplication removal, towards the \task\ task. Our data and code are publicly available.\footnote{\url{https://github.com/megagonlabs/qa-summarization}}
%also reveal that \tingyao{using pretrained language models in a multi-task manner do (1) reduce the duplicated problem in CQA (2) sentence-style transfer } \todo{key findings here}. Our data and code are available at \codeurl. 

% \kenneth{I would try to emphasize why the task is needed. People know Amazon platform is important and CQA is an very old/well-developed research area. BUT why do we need summary? I also rewrote the abstract a bit.}
% \tingyao{Show some examples to emphasize that data is noisy and mention in the paragraph}

% Millions of questions are asked and answered on online e-commerce sites daily.
% The large volume of QAs could easily overwhelm users, especially when they want to know the key information but do not have particular questions in mind.
% To help users quickly digest information in QAs, we propose a novel \task task that aims at producing a concise and declarative summary of the key information in the QAs.\kenneth{What does ``declarative'' mean here? This word is not very clear. What do we want to say?}
% We create a new benchmark dataset, \corpus, that contains human-written summaries based on the QA pairs of 1,440 products on Amazon.
% We also establish a set of strong baselines, including both extractive and abstractive summarization models, showing the challenging nature of the \task task.
% \kenneth{I would add one sentence to describe one key results here. BLEU? Human evaluation? You should describe the eval result.}\tingyao{mention some evaluation results here}
% Our data and code are available at \codeurl.



==> EMNLP-2022 CoQASum/sections/analysis.tex <==
%\tingyao{one details, one for performance}
%\subsection{Domain Transfer}
%To see if our intended framework can be adapted to different domains, we treat each category as a separate domain. We first fine-tune the models on one category before applying the pretrained models to other categories to see if the information can be transferred between them. \tingyao{say something according to the results}

%\subsection{Different Pre-trained Models}
\subsection{Choice of Pre-trained Language Models}
To justify our observation that pre-trained language models have strong abilities 
%to reduce redundancy and perform sentence-type transfer,
we test and compare three additional pre-trained language models on \corpus: PEGASUS~\cite{zhang2020pegasus}, T5~\cite{raffel2020exploring}, and BART~\cite{lewis2019bart}.
%
We confirm that all models perform better than the extractive and extractive-abstractive models. While PEGASUS and T5 show similar ($24.81$ and $24.61$ RL, respectively), they are less effective than BART and LED ($26.89$ and $26.01$ RL, respectively).
%To further justify our observation that pre-trained language models have strong abilities to reduce redundancy and perform style transfer, we further test and compare three additional pre-trained language models: PEGASUS~\cite{zhang2020pegasus}, T5~\cite{raffel2020exploring}, BART~\cite{lewis2019bart}. We observe that all variation of pre-trained langauge models show better performance than extractive or extractive-abstrative methods. While PEGASUS and T5 shows similar ($24.81$ and $24.61$ RL respectively), they are less effective than BART and LED ($26.89$ and $26.01$ RL respectively). %\xiaolan{cannot salvage generated summaries to re-run evaluation. Let's skip the detailed results}

%Although we demonstrate that language models have a strong ability to reduce redundancy and perform style transfer on the QA summarization task, we are unsure whether they perform well in an abstractive manner in general. To investigate the effect of pretrained datasets further, we compare several cutting-edge pretrained language models. All models are fine-tuned on our QA dataset. All models have competitive performance, with BART outperforming the other three. The overall performance is shown in \Cref{tab:result-pretrained-model}.

\iffalse

\begin{table}[t]
    \small
    % \centering
    \begin{tabular}{l|rrrr}
    \toprule 
    & \multicolumn{1}{c}{R1} & \multicolumn{1}{c}{R2} &  \multicolumn{1}{c}{RL} & \multicolumn{1}{c}{BS} \\ \midrule
     PEGASUS & 45.28 & 18.00 & 24.81 & 25.47 \\
     T5 & 44.56 & 17.62 & 24.61 & \\
     BART & 48.19 & 21.13 & 26.89 &  \\
     LED & 45.82 & 19.34 & 26.01 & \\
     \bottomrule
    \end{tabular}
    \caption{Different pretrained model result}
    \label{tab:result-pretrained-model}
\end{table}
\fi

%\subsection{Limited Training Data}
\subsection{Learning Curve Analysis}
Since collecting reference summaries is costly and time-consuming, we investigate the models' performance with limited training data. We tested the models' performance when trained with 20\%, 40\%, \dots, 100\% of the training data.
%
Figure~\ref{fig:lowratio} shows the ROUGE-L F1 scores of \model{} and FastAbstractiveSum when trained on different size of training data. 
%
By leveraging a pre-trained checkpoint, \model{} performs consistently and substantially better than FastAbstractiveSum, which is trained from scratch. 
%
\model{} also shows a faster learning curve and reaches the plateau in performance when trained with 60\% and more data. This supports that the annotation size of \corpus{} is sufficient for fine-tuning pre-trained language models, while it may be insufficient for non-pre-trained models.

%\xiaolan{Add results with 20\%, 40\%, 60\%, 80\% of training data. } \tingyao{put result into line chart}
%Since performing summary annotation is a costly and time-consuming process, we further investigate models performance w.r.t limited training data. In particular, we reduce the ratio of training examples up to $20\%$ and tested the models' performance. As shown in Figure~\ref{fig:lowratio}, reducing ratio of training examples significantly decrease the models performance, which aligns with our expectation. At the same time, leveraging pre-trained checkpoints, DedupLED performs consistently and substantially better than FastAbstractiveSum, which is trained from scratch. 
%\tingyao{I can update the linechart once you have result} \xiaolan{to continue}. 

%We wanted to see how much the limited data would affect performance, so we experimented with different numbers of QA pairs to fine-tune the models. Results show in \Cref{tab:result-different-ratio}. The size of data is still important for our task as the performance get better as the size increase. \tingyao{say something according to the results}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{fig/input_ratio.pdf}
    \caption{Learning curve analysis. $x$-axis is the training data ratio, and $y$-axis is the performance on the test set.}
    %\caption{Different ratio of training data. %\tingyao{update 60, 80 results}}
    \label{fig:lowratio}
\end{figure}

% \begin{table*}[t]
%     \centering
%     \begin{tabular}{lrrrrrrr}
%     \toprule \hline
%     Models & \multicolumn{1}{c}{data} & \multicolumn{1}{c}{R1-F} &  \multicolumn{1}{c}{R2-F} &  \multicolumn{1}{c}{RL-F} &  \multicolumn{1}{c}{BERT-F} \\ \hline
%     \multirow{4}{*}{FastAbstractiveSum}&20\%&32.44&7.09&17.33&82.05 \\
%      & 40\% & 35.14 & 9.40 & 18.94 & 83.10 \\
%      & 60\% & 39.79 & 12.04 & 20.93 & 83.87 \\
%      & 80\% & 36.49&10.78&20.40&84.11 \\ \hline
%     \multirow{4}{*}{model 2} &20  \\
%      & 40 &  \\
%      & 60 & \\
%      & 80 &  \\
%      \hline \bottomrule
%     \end{tabular}
%     \caption{Different ratio of training data\todo{To be updated, check 80\%}}
%     \label{tab:result-different-ratio}
% \end{table*}


%\subsection{Cross-category transfer learning ability}
\subsection{Cross-category Transfer Learning}
\corpus{} contains 17 different categories and varying amounts of entities within each category.
%
To investigate how different categories and numbers of training data affect the summarization performance, we experiment DedupLED on the top five categories in terms of entity count. We first fine-tuned DedupLED on each category and tested it on the five categories. For each category, we split entities into train/dev/test sets in 0.8/0.1/0.1 ratios.


Table~\ref{tab:cross-category2} shows ROUGE-1 F1 scores of the DedupLED models in a cross-category setting. 
%
We find that more training data generally helps improve the model quality even if not fine-tuned on training data in the same category. Electronics and Home \& Kitchen are the top two categories with the most training examples (243 and 209 entities, respectively), and achieved the best performance across all categories. 
%They even achieved comparable performances when compared to those trained on the entire dataset. \xiaolan{I removed this because we did not show per-category performance with model trained on entire dataset}
%On the other hand, we observe that DedupLED models fine-tuned on categories with a smaller amount of training data still shows solid performance. 
%
From the results, we confirm that
%Furthermore, we confirm that 
summarization models based on pre-trained language models
%, such as DedupLED, \yoshi{it's a little bit overclaimed as we only tested DedupLED. Let's not refer to DedupLED and overclaim it. :p}
have strong cross-category transfer ability in \task.

% \begin{table*}[t]
% \scriptsize
%     \centering
%     \begin{tabular}{l|ccc|ccc|ccc|ccc|ccc}
%     \toprule  
%     & \multicolumn{3}{c|}{\textbf{Electronics}} 
%     & \multicolumn{3}{c|}{\textbf{Home and Kitchen}}
%     & \multicolumn{3}{c|}{\textbf{Sports and Outdoors}} 
%     & \multicolumn{3}{c|}{\textbf{Tools and Home.}}
%     & \multicolumn{3}{c}{\textbf{Automotive}} \\
%     & \multicolumn{1}{c}{R1} & \multicolumn{1}{c}{R2} &  \multicolumn{1}{c|}{RL} & 
%     \multicolumn{1}{c}{R1} & \multicolumn{1}{c}{R2} &  \multicolumn{1}{c|}{RL} &
%     \multicolumn{1}{c}{R1} & \multicolumn{1}{c}{R2} &  \multicolumn{1}{c|}{RL} &
%     \multicolumn{1}{c}{R1} & \multicolumn{1}{c}{R2} &  \multicolumn{1}{c|}{RL} &
%     \multicolumn{1}{c}{R1} & \multicolumn{1}{c}{R2} &  \multicolumn{1}{c}{RL}\\ \midrule
%     \textit{Pretrained domain:} & &&&&&&&&&&&\\
%      \quad Electronics 
%      & 46.75 & 22.73 & 24.40 
%      & 41.74 & 18.28 & 24.26 
%      & 46.92 & 23.91 & 26.58
%      & 38.90 & 17.65 & 24.16
%      & 40.52 & 15.36 & 20.78 \\
%      \quad Home and Kitchen 
%      & 41.84 & 17.53 & 22.04
%      & 41.97 & 16.68 & 24.25 
%      & 44.46 & 20.20 & 23.61
%      & 37.51 & 15.96 & 22.99
%      & 42.53 & 15.55 & 22.76 \\
%      \quad Sports and Outdoors 
%      & 38.26 & 13.79 & 21.51 
%      & 42.99 & 17.88 & 21.93 
%      & 38.64 & 15.74 & 21.89
%      & 39.17 & 13.25 & 21.78
%      & 36.18 & 16.25 & 20.79 \\
%      \quad Tools and Home. 
%      & 42.86 & 18.47 & 23.15 
%      & 40.50 & 14.21 & 21.85 
%      & 40.25 & 17.35 & 22.22
%      & 38.40 & 19.08 & 21.20
%      & 38.05 & 13.76 & 19.83 \\
%      \quad Automotive 
%      & 41.71 & 17.50 & 22.94 
%      & 38.96 & 13.09 & 22.53
%      & 40.34 & 16.82 & 23.36
%      & 38.75 & 17.92 & 24.33
%      & 37.53 & 12.70 & 20.26 \\
%      \bottomrule
%     \end{tabular}
%     \caption{Zero-shot performance of \model{} on top-5 cross-category. R1/R2/RL/ denotes ROUGE-1/2/L F1 scores, respectively. Pretrained in one domain with more entities would perform much better cross-domain in general.}
%     \label{tab:cross-category}
% \end{table*}

\begin{table*}[t]
% \large
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c|c}
    \toprule  
    &&\multicolumn{5}{c|}{{\bf Test category}} \\
    {\bf Training category} & {\bf |Train|}
    % & {\bf |Val|} & {\bf |Test|}
    & \multicolumn{1}{c|}{ELEC}
    & \multicolumn{1}{c|}{H\&K}
    & \multicolumn{1}{c|}{S\&O}
    & \multicolumn{1}{c|}{T\&H}
    & \multicolumn{1}{c|}{AUTO}
    & \multicolumn{1}{c}{\bf Avg }\\\midrule
% \textit{Training domain:} & & & & &\\
     \quad ELEC 
     & 243 
    %  & 30 & 31
     & {\bf 46.75}
     & 41.74
     & {\bf 46.92}
     & 38.90
     & 40.52
     & \multicolumn{1}{c}{{\bf 42.97}} \\
     \quad H\&K 
     & 209 
    %  & 26 & 27 
     & 41.84
     & {\bf 41.97}
     & 44.46
     & 37.51
     & {\bf 42.53} 
     & \multicolumn{1}{c}{41.66}\\
     \quad S\&O
     & 130 
    %  & 16 & 17 
     & 38.26
     & 42.99 
     & 38.64
     & {\bf 39.17}
     & 36.18 
     & \multicolumn{1}{c}{39.05} \\
     \quad T\&H 
     & 110 
    %  & 14 & 14
     & 42.86
     & 40.50 
     & 40.25
     & 38.40
     & 38.05 
     & \multicolumn{1}{c}{40.01} \\
     \quad AUTO 
     & 76 
    %  & 9 & 10
     & 41.71 
     & 38.96
     & 40.34
     & 38.75
     & 37.53 
     & \multicolumn{1}{c}{39.46} \\
     \bottomrule
    \end{tabular}
    \caption{Cross-category performance (ROUGE-1 F1) of \model{} on top-5 product categories: Electronics (ELEC), Home and Kitchen (H\&K), Sports and Outdoors (S\&O), Tools and Home (T\&H), and Automatic (AUTO). Each model was trained on training data of each category and then tested on the five categories. The highest ROUGE-1 F1 scores for each category are bold-faced.}
    \label{tab:cross-category2}
\end{table*}

\iffalse
\begin{table*}[t]
\scriptsize
    \centering
    \begin{tabular}{l|c|c|c|c|c}
    \toprule  
    & \multicolumn{5}{c}{{\bf Test category (R1/R2/RL)}} \\
    {\bf Training category (|train|)}
    & \multicolumn{1}{c}{Electronics}
    & \multicolumn{1}{c}{Home and Kitchen}
    & \multicolumn{1}{c}{Sports and Outdoors}
    & \multicolumn{1}{c}{Tools and Home}
    & \multicolumn{1}{c}{Automotive} \\\midrule
% \textit{Training domain:} & & & & &\\
     \quad Electronics (304)
     & {\bf 46.75}/{\bf 22.73}/{\bf 24.40}
     & 41.74/{\bf 18.28}/{\bf 24.26}
     & {\bf 46.92}/{\bf 23.91}/{\bf 26.58}
     & 38.90/17.65/24.16
     & 40.52/15.36/20.78 \\
     \quad Home and Kitchen (264) 
     & 41.84/17.53/22.04
     & {\bf 41.97}/16.68/24.25
     & 44.46/20.20/23.61
     & 37.51/15.96/22.99
     & {\bf 42.53}/15.55/{\bf 22.76} \\
     \quad Sports and Outdoors (163)
     & 38.26/13.79/21.51 
     & 42.99/17.88/21.93 
     & 38.64/15.74/21.89
     & {\bf 39.17}/13.25/21.78
     & 36.18/{\bf 16.25}/20.79 \\
     \quad Tools and Home (138) 
     & 42.86/18.47/23.15 
     & 40.50/14.21/21.85 
     & 40.25/17.35/22.22
     & 38.40/{\bf 19.08}/21.20
     & 38.05/13.76/19.83 \\
     \quad Automotive (95)
     & 41.71/17.50/22.94 
     & 38.96/13.09/22.53
     & 40.34/16.82/23.36
     & 38.75/17.92/{\bf 24.33}
     & 37.53/12.70/20.26 \\
     \bottomrule
    \end{tabular}
    \caption{\hll{Cross-category performance of \model{} on top-5 product categories. Each model was trained on training data of each category and then tested on the five categories. R1/R2/RL/ denotes ROUGE-1/2/L F1 scores, respectively. The highest ROUGE scores for each category are bold-faced. Note that different categories have different numbers of entities for training, as shown in (). }\todo{Ting-Yao: what is the train/dev/test split in this experiment, can you update # of entities to reflect this?}}
    \label{tab:cross-category}
\end{table*}
\fi


% \begin{table}[]
% \small
%     \centering
%     \begin{tabular}{l|c|c|c}
%     \toprule
%     & Inf. & Coh. & Con. \\ \midrule
%     Electronics (304 entities) &-8.41&-5.72&-8.42 \\
%     Home and Kitchen (264 entities)
%     &-4.71&+1.01&+3.37 \\
%     Sports (163 entities)
%     &-2.02&-6.07&-1.35 \\
%     Tools (138 entities)
%     &+13.13&+5.72&+4.38\\
%     Automotive (95 entities)
%     &+13.13&+5.72&+4.38\\\bottomrule
%     \end{tabular}
%     \caption{Performance of top-5 cross-category.}
%     \label{tab:cross-category}
% \end{table}

% \tingyao{probably not enough time, Q-only input, A-only input}



==> EMNLP-2022 CoQASum/sections/conclusion.tex <==
%\todo{sum up}
%In this paper, 
We propose the \task\ task to summarize QA pairs in Community-based Question Answering. 
%
We develope a multi-stage annotation framework and created a benchmark \corpus{} for the \task\ task. Our multi-stage annotation framework decomposes a complex annotation task into three much simpler ones, thus allows higher annotation quality. We further compare a collection of extractive and abstractive summarization methods and establish a strong baseline method DedupLED for the \task\ task. Our experiment also confirms two key challenges, sentence-type transfer and duplication removal, towards the \task\ task. 

%
%The annotation pipeline first selects representative QA pairs and rewrites them into declarative sentences before rewriting them into final reference summaries. We also enriched the QAs to mimic real-word scenario. \yoshi{enrichment is missing here.}

% The comparative experiments confirmed that the two factors, (1) duplicate removal and (2) sentence-type transfer, are essential to solving the task.

%We conduct comparative experiments to confirm it is essential to do (1) duplicate removal and (2) sentence-type transfer to solve the task. We further set up a strong baseline, DedupLED, \tingyao{emphasize again}

%\yoshi{Take 1. Is super awkward. Feel free to edit/rewrite from scratch. Better than nothing.}


\section*{Limitations}
%\tingyao{ EMNLP 2022 requires all papers to have a clear discussion of limitations, in a dedicated section titled “Limitations”. This section will appear at the end of the paper, after the discussion/conclusions section and before the references, and will not count towards the page limit. Papers without a limitation section will be automatically rejected without review.}

% 
% Mandatory Discussion of Limitations
%
% We believe that it is also important to discuss the limitations of your work, in addition to its strengths. EMNLP 2022 requires all papers to have a clear discussion of limitations, in a dedicated section titled “Limitations”. This section will appear at the end of the paper, after the discussion/conclusions section and before the references, and will not count towards the page limit. Papers without a limitation section will be automatically rejected without review.
%
% ARR-reviewed paper that did not include “Limitations” section in their prior submission, should submit a PDF with such a section together with their EMNLP 2022 submission.
%
% While we are open to different types of limitations, just mentioning that a set of results have been shown for English only probably does not reflect what we expect. Mentioning that the method works mostly for languages with limited morphology, like English, is a much better alternative. In addition, limitations such as low scalability to long text, the requirement of large GPU resources, or other things that inspire crucial further investigation are welcome.

As we propose and tackle a challenging summarization task, the paper has certain limitations. First, our benchmark is in a single domain (E-commerce) in a single language (English), %\tingyao{there are few Spanish QAs},
which not necessarily ensuring the generalizability for other domains and languages. 
%
Second, the quality of our annotations relies on the initial selection of seed QA pairs. As we discussed in the paper, we filtered high-quality seed QA pairs to minimize the risk. Nevertheless, it may not accurately replicate the summarization procedure by experts.
%
Third, we use rules and heuristics to ensure the quality of the free-text annotation. Despite being able to detect and eliminate a significant ratio of low-quality annotation, our rules and heuristics do not provide perfect guarantee, meaning that \corpus{} may still contain noisy and low-quality annotations.  
%
With those limitations, we still believe that the paper and the benchmark are benefitial for the community to take a step beyond the scope of existing summarization tasks. 

\section*{Ethics Statement}
For the annotation tasks, we paid \$10 hourly wage for the crowd workers on MTurk and Appen (Steps 1 and 3) and $\$15$ to $\$30$ hourly wage for the Upwork contractors (Step 2), making sure to pay higher than the minimum wage in the U.S. (i.e., \$7.25 per hour). 
%
Our \corpus{} is based on the publicly available Amazon QA dataset. To our knowledge, the dataset does not contain any harmful content.
%In the rewriting task, we pay \$10 hourly pay for the crowd workers on Mturk (Sub-task 1) and $\$15$ to $\$30$ hourly pay for Upwork contractors (Sub-task 2). Our \corpus{} is based on public Amazon QA dataset and does not contain any harmful content.
% \tingyao{not sure if we have the issue, if not, just ignore}
% \yoshi{Mention payment for crowd-sourced workers and the corpus does not contain any harmful content, I guess?}

% \begin{itemize}
%     \item English-only
%     \item E-commerce only (Amazon)
%     \item Sampling bias caused by the choice of the seed QA pairs
% \end{itemize}



==> EMNLP-2022 CoQASum/sections/corpus.tex <==


% https://docs.google.com/drawings/d/108Wb-et2Jh9pGik9WB1AS8hnDLGnrJm1Lc9RVWrVDzM/edit?usp=sharing
\begin{table*}[h]
\small
\centering
\begin{tabular}{l|r|rrr|rrrr}
\toprule
\multirow{2}{*}{\textbf{Category}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{|Entity|}}} & %\multicolumn{3}{c|}{\textbf{Input/Raw Sum./Gold Sum.}} &
\multicolumn{3}{c|}{\textbf{Avg. word count}} &
\multicolumn{4}{c}{\textbf{\% of novel n-grams in gold summary}}
% \multicolumn{2}{c}{\textbf{Max. words}} & \multicolumn{2}{c}{\textbf{Med. words}}
\\ 
% \cline{3-10}
     &  & 
    %  \multicolumn{1}{c}{\textbf{Total Num.}} &
     %\multicolumn{3}{c|}{\textbf{length}} &
      \multicolumn{1}{c}{\textbf{Input}} & 
      \multicolumn{1}{c}{\textbf{Raw sum.}} &
      \multicolumn{1}{c|}{\textbf{Ref sum.}} &
      %
      \multicolumn{1}{c}{\textbf{unigram}} &
      \multicolumn{1}{c}{\textbf{bigram}} &
      \multicolumn{1}{c}{\textbf{trigram}} & 
      \multicolumn{1}{c}{\textbf{4-gram}}
     \\ \midrule
% Automotive & 95 &1044.77&167.08&117.25&21.16&57.80&75.43&83.37 \\
% Baby & 17 & 1162.65&156.41&113.70&28.56&69.56&86.09&92.69 \\
% Beauty & 20 & 1038.45&161.2&127.23&23.96&62.84&81.82&89.15 \\
% Cell Phones and Accessories & 94 & 931.47&135.8&96.48&16.24&50.56&69.07&78.18 \\
% Clothing Shoes and Jewelry & 10 & 1134.80&159.3&130.18&16.67&48.17&64.81&72.92\\
% Electronics &304 &1000.58&167.26&132.09&22.06&55.11&70.73&77.77 \\
% Grocery and Gourmet Food & 22 & 908.41&123.41&96.68&16.17&54.91&74.52&82.81 \\
% Health and Personal Care & 80 & 1125.74&139.64&103.64&15.42&52.75&71.10&79.74 \\
% Home and Kitchen & 262 & 1093.63&153.19&113.46&23.00&62.04&79.08&86.21 \\
% Musical Instruments & 22 & 899.95&196.95&142.05&35.06&66.65&78.40&82.85 \\
% Office Products & 66 & 994.33&141.41&103.73&12.69&45.20&63.21&72.94 \\
% Patio Lawn and Garden & 70 & 1177.17&142.1&107.49&12.92&47.08&65.16&74.80 \\
% Pet Supplies & 11 & 1154.91&124.82&106.54&16.51&53.42&73.91&83.84\\
% Sports and Outdoors &163 &1119.97&143.72&106.37&13.85&47.57&66.26&75.65 \\
% Tools and Home Improvement & 138&1095.97&167.57&109.95&18.68&45.58&58.63&65.07\\
% Toys and Games & 54 & 984.65 &150.17 & 112.32&21.41&60.85&79.28&86.94 \\
% Video Games&12&1087.58&186.42&128.67&28.59&61.22&76.87&83.70 \\
Automotive & 95 & 1044.8 & 167.1 & 117.3 & 21.16&57.80&75.43&83.37 \\
Baby       & 17 & 1162.7 & 156.4 & 113.7 & 28.56&69.56&86.09&92.69 \\
Beauty     & 20 & 1038.5 & 161.2 & 127.2 &23.96&62.84&81.82&89.15 \\
Cell Phones and Accessories & 94 & 931.5 & 135.8 & 96.5 & 16.24&50.56&69.07&78.18 \\
Clothing Shoes and Jewelry & 10 & 1134.8 & 159.3 &130.2 & 16.67&48.17&64.81&72.92\\
Electronics & 304 & 1000.6 & 167.3 & 132.1 & 22.06&55.11&70.73&77.77 \\
Grocery and Gourmet Food & 22 & 908.4 & 123.4 & 96.7 &16.17&54.91&74.52&82.81 \\
Health and Personal Care & 80 & 1125.7 & 139.6 & 103.6 &15.42&52.75&71.10&79.74 \\
Home and Kitchen & 262 & 1093.6 & 153.2 & 113.5 & 23.00&62.04&79.08&86.21 \\
Musical Instruments & 22 & 900.0 & 197.0 & 142.1 & 35.06&66.65&78.40&82.85 \\
Office Products & 66 & 994.3 & 141.4 & 103.7 & 12.69&45.20&63.21&72.94 \\
Patio Lawn and Garden & 70 & 1177.2 & 142.1 &107.5 & 12.92&47.08&65.16&74.80 \\
Pet Supplies & 11 & 1154.9 & 124.8 & 106.5 & 16.51&53.42&73.91&83.84\\
Sports and Outdoors &163 & 1120.0 & 143.7 &106.4 &13.85&47.57&66.26&75.65 \\
Tools and Home Improvement & 138&1096.0 & 167.6 & 110.0 &18.68&45.58&58.63&65.07\\
Toys and Games & 54 & 984.7 & 150.2 & 112.3 &21.41&60.85&79.28&86.94 \\
Video Games & 12 & 1087.6 & 186.4 & 128.7 & 28.59&61.22&76.87&83.70 \\
\midrule
%\textbf{All} & 1,440 & 1055.55 & 154.77 & 114.79&19.46&54.17&71.06&78.88
\textbf{All} & 1,440 & 1055.6 & 154.8 & 114.8& 19.46&54.17&71.06&78.88
\\ \bottomrule
\end{tabular}
 \caption{\corpus{} 
%  Our Amazon QA 
 dataset statistics. %Input/Raw Sum./Gold Sum. length refer to the average number of tokens in the input, raw summary (formed by rewritten seed QAs), and gold-standard summary, respectively.
 %\url{https://aclanthology.org/W19-8665.pdf} \tingyao{updated scores done}  
 }
\label{tab:qa_dataset-stats}
\end{table*} 



%\subsection{Original Amazon QA dataset}
We first describe the multi-stage annotation framework to collect gold-standard reference summaries from input QA pairs and then describe our benchmark dataset \corpus.
%, which is built from the public Amazon CQA dataset~\cite{wan2016modeling,mcauley2016addressing}. 


\subsection{A Multi-stage Annotation Framework}\label{sec:annotation}
Reading and summarizing a set of QA pairs is challenging and error-prone for three reasons: (1) a large number of QA pairs, (2) the heavy repetition and noise in both questions answers, and (3) the difficulty of converting questions and answers into declarative summaries.
%
Thus, it is infeasible to collect high-quality reference summaries by simply showing a set of QA pairs and asking annotators to write a summary.
%
In this paper, we design a multi-stage annotation framework that first simplifies this complex annotation task into more straightforward annotation tasks and then enriches the collected annotations.


Figure~\ref{fig:annotation} depicts the schematic procedure of the multi-stage annotation framework.
%
For each entity and its corresponding QA pairs in the original corpus, we first select representative seed QA pairs and ask annotators to rewrite them into declarative sentences, which are then concatenated into a raw summary. 
%
Next, we ask highly-skilled annotators to polish the raw summary into a more fluent summary. 
%
In the last step, we enrich the seed QA pairs by selecting semantically similar QA pairs from the original corpus.

% Asking human annotators to read and summarize a set of questions and answers is a challenging and error-prone process because (1). the large number of QA pairs; (2). the heavy repetition and noise in both questions an answers; (3). the difficulty of converting question and answers into plain text. As a result, it is infeasible to obtain a high-quality dataset by simply showing a set of QAs and asking annotators to write a summary. In this paper, we present a multi-stage annotation framework that decomposes this complex annotation task into three easier sub-tasks. Given an entity and its QA corpus, we first select a set of non-redundant (or less-redundant) QAs as the seed and then ask annotators to post-edit the seed QAs into plain text. Next, we asked high-skilled annotators to further summarize and polish the post-edited QAs into a fluent summary. Finally, we further enrich the seed QAs as the input by selecting semantically similar QAs from the entity's QA corpus.
% %
% Figure~\ref{fig:annotation} depicts the schematic procedure of the multi-stage annotation framework.

%\subsubsection*{Sub-task 1: Select and Rewrite Seed QAs}
\subsubsection*{Step 1: QA Pair Selection and Rewriting}
%Writing a summary directly from a large set of repetitive QAs is extremely challenging since it is already hard to trace whether the summary covers all the key information in the input, not to mention the difficulty of writing a paragraph of coherent and fluent text. Thus, instead of using a single-step annotation task, 
% In this sub task, we use a very aggressive strategy to perform the QA de-duplication and further ease the summary writing task by asking annotators to rewrite pairs of question and answer into plain text. 
% A natural way to de-duplicate QAs is by comparing the semantics of existing QAs and only keep the unique ones. However, we found that this approach less practical because asking human annotators to perform the comparison is extremely costly. In addition, it is hard to validate the quality because selecting a representative QA out of a set of semantically similar ones is a very subjective process. Thus, we take a heuristic-based strategy to aggressively select non-duplicated seeds from the QA corpus instead. In particular, we first use rules to filter-out QAs that are likely in lower quality and then randomly sample $k$\footnote{We set $k=8$ for \corpus.} seed QAs from the remaining ones. 
% More specifically, based on our observations we use the following two rules to filter-out low quality QAs: (1). \textit{length rule}: QAs with less than $5$ or more than $150$ tokens; (2). \textit{pronoun rule}: QAs that include first person pronouns. In addition, to avoid redundancy, we only sample seed QAs of different questions. 

% To further ease the annotation process, we ask crowd-sourcing annotators to rewrite the selected seed QAs into declarative sentences (i.e., plain text). In particular, we recruit three crowd
% workers from Amazon Mechanical Turk to rewrite every representative QA pair. In addition, we adapt a series of rules, e.g., forbidden direct copy of the original QA or use first person pronouns, to ensure the quality of the rewritten QAs. The interface and rules of the annotation task can be found in Appendix~\ref{sec:appendix:post-edit}. Note that we further use such rules to quantify the quality of the annotated QAs and only include the best one for the next sub-task. 
%% Background
In this step, we use a drastic strategy to remove duplicate QA pairs and simplify the annotation task for human annotators. 
%
A natural way to deduplicate QA pairs is by manually comparing existing QA pairs' semantics and only keeping the unique ones. However, we found this approach less practical because asking human annotators to perform the comparison is extremely expensive. It is also hard to validate the quality because selecting a representative QA from a set of semantically similar ones is a subjective process.

%% Heuristics
Thus, we use a heuristic-based strategy to select representative QA pairs from the original corpus. 
%
Specifically, we use the following two rules to filter out QA pairs that are not suitable for creating reference summaries: (1) \textit{length rule}: QA pairs with less than $5$ or more than $150$ tokens;
%\yoshi{The total word count of a QA pair?} \xiaolan{yes}
(2) \textit{pronoun rule}: QA pairs that include first-person pronouns. We found that long questions/answers tend to contain their background information (e.g., personal stories), which is irrelevant to the entity. First-person pronouns are also a strong indicator for such questions/answers.
%
After the filtering, we randomly sample $k$ seed QA pairs from the remaining ones. In addition, to avoid redundancy, we only sample seed QA pairs of different questions.\footnote{Note that there is a chance that selected QA pairs contain duplicate information. We make sure to exclude such duplicate information in Step 2.}

%% Annotation task
For each of the $k$ seed QA pairs, we ask human annotators to rewrite them into declarative sentences. We recruited three crowd workers from Amazon Mechanical Turk\footnote{\url{https://www.mturk.com/}} to annotate every QA pair and chose the highest-quality annotation based on 6 criteria: (1) length of LCS against the original QA pair, (2) use of yes/no, (3) use of interrogative determiner (e.g., What), (4) use of first-person pronouns, (5) use of the item name at the beginning, (6) the ignorance of the question information. We also blocked MTurk workers with consistently low-quality annotations to ensure the quality of annotations.
%for this rewriting task.
%
% [original] In addition, we adopt a series of rules (e.g., forbidden direct copy of the original QA or the use of first-person pronouns) to ensure the quality of the rewriting process. We further use those rules to quantify the quality of the annotations and select the best one for the next step. 
%The task interface and rules of the annotation task can be found in Appendix~\ref{sec:appendix:post-edit}. 

%we asked 3 MTurk workers to annotate every QA pair and chose the highest-quality annotation based on 6 criteria described in LL210-212. The criteria are (1).length of LCS against the original QA pair, (2).use of yes/no, (3).use of interrogative determiner (e.g., What), (4).use of first-person pronouns, (5).use of the item name at the beginning, (6).the ignorance of the question information. We also blocked MTurk workers with consistently low-quality annotations to ensure the quality of annotations.


%\subsubsection*{Sub-task 2: Write Gold-standard Summary}
\subsubsection*{Step 2: Summary Writing}
% From the first sub-task, we obtained the rewritten seed QAs in declarative sentences. We further use them to form the raw summary by simply concatenating the best quality one.  
% %By concatenating the post-edited QAs, we form the raw summary of the corresponding entity. 
% However, we noticed that the raw summaries are not very fluent and may still contain redundant information. To address these issues, we use an another crowd-sourcing task to further polish the raw summary. To ensure the quality, we hired high-skilled annotators from  Upwork~\footnote{\url{https://www.upwork.com/}} to accomplish this task. For each entity, we only show annotators to write the raw summary into a fluent and succinct gold-standard summary. Detailed interface of this task can also be found at Appendix~\ref{sec:appendix:post-edit}.
We form a raw summary by concatenating annotations (i.e., declarative sentences rewritten from QA pairs) obtained in the first step for each entity.
%
The raw summaries are not necessarily fluent and coherent as different pieces are annotated independently. They may also contain redundant information. 
%
To address these issues, we use another annotation task to polish and write a summary from the raw summary. To ensure the quality, we hired highly-skilled writers from  Upwork\footnote{\url{https://www.upwork.com/}} by conducting screening interviews for this annotation task.
%
For each entity, we show annotators the raw summary and ask them to write a fluent and concise summary. %The detailed interface of this task can also be found in Appendix~\ref{sec:appendix:post-edit}.



%\subsubsection*{Sub-task 3: Enrich the Input QAs}
\subsubsection*{Step 3: Enriching Input QA Pairs}
% Recall that in Sub-task 1, we select $k$ seed QAs for the summary annotation. The seed QAs are less redundant because of our aggressive filtering and sampling strategy. However, the seed QAs may not represent the real-world scenario, where similar questions are asked multiple times and each question often contains several answers. To make our benchmark closer to the realistic settings, our last sub-task focuses on enriching the selected seed QAs. 
% In particular, we first include all the answers to the questions of the seed QAs (or seed questions). Besides, we also include questions, which are semantically similar to the seed questions, and all their answers as part of our input. To retrieve semantically similar questions, we use BERT embeddings and word overlap to find the candidates, followed by an additional crowd-sourcing task for further validation. The validation step ensures that our gold-standard summaries are also applicable for the enriched set of QAs. 
Recall that in Step 1, we select $k$ seed QA pairs for each entity. The seed QA pairs are less redundant because of the filtering and sampling strategy. This does not reflect the real-world scenario, where similar questions are asked multiple times, and each question often contains several answers.

To align the benchmark with more realistic settings, we enrich the input QA pairs in Step 3. 
%
In particular, we add all answers to every question in the seed QA pairs. Besides, we retrieve questions that are semantically similar to seed questions and add all the answers to the input QA pairs. For semantic similarity calculation, we use BERT embeddings and word overlap to find the candidates, followed by an additional crowd-sourcing task using Appen\footnote{\url{https://appen.com/}} for manual validation.
%
The validation step ensures that our reference summaries can be created from the enriched input QA pairs.
%\tingyao{do we want to mention how many numbers of enriched data we collect?} \xiaolan{I think it is OK to skip.}\yoshi{+1}




%\subsection{The \corpus\ Dataset}
\subsection{Dataset Statistics}
%\yoshi{The subsection title was similar to the section title}
%Following the multi-stage annotation framework, we created the \corpus\ benchmark dataset from the Amazon QA dataset~\cite{wan2016modeling,mcauley2016addressing}. We select $1,440$ entities from $17$ categories with $39,485$ QAs and obtained $1440$ gold-standard summaries. Besides, from Sub-task 1, we also obtained an annotated dataset that rewrite individual QA into declarative sentences. This additional annotated dataset contains $11,520$ QAs, each of which has $3$ annotations. 
Using the multi-stage annotation framework, we created the \corpus\ benchmark based on the Amazon QA dataset~\cite{wan2016modeling,mcauley2016addressing}.
%
We selected 1,440 entities from 17 product categories with 39,485 input QA pairs and 1,440 reference summaries. Besides, \corpus{} also contains rewritten QA pairs in declarative sentences for the QA pair rewriting task in Step 1, which consist of 3 annotations for each of the 11,520 seed QA pairs ($k=8$ seed QA pairs for each entity). 

%In summary, we obtained \todo{$1,440$} gold-standard summaries and  \tingyao{including different annotator or only best post-edited from original 8 seed QAs?} \todo{$11,520$} post-edited QAs from sub-task 1. Detailed statistics of \corpus\ can be found in Table~\ref{tab:qa_dataset-stats}.

% \yoshi{We should justify the quality of the dataset by referring to the numbers in the table.}

% %% Summary length < Raw summary length
% As the final summary length is shorter than the raw summary (i.e., the concatenation of the 8 seed QA pairs written in declarative sentences), we confirm that the final summary rewriting task makes sure to remove redundant information spread over sentences created from different QA pairs. 

% %% The compression rate
% The average input-summary length is 9.2, which is \todo{compare against other summarization datasets. Answer Summarization and EmailSumm, for example?}

% %% Abstractiveness
% The novel n-gram ratio of the reference summary indicates that the benchmark offers a fairly abstractive summarization task. The numbers are close to the XSum dataset~\cite{narayan-etal-2018-dont}, which is known to be among the most abstractive summarization datasets. 

Table~\ref{tab:qa_dataset-stats} shows the statistics of \corpus. 
%
We confirm that the average word count of input QA pairs/raw summaries/reference summaries is consistent for different categories.
%
%% Novel-ngram
The novel n-gram distributions also confirm that \corpus{} offers a fairly abstractive summarization task. Some product categories such as ``Office Products'' and ``Patio Lawn and Garden'' have lower novel n-gram ratios, indicating that the task becomes relatively extractive. %\yoshi{Any insights about it?}
%
%% Summary length < Raw summary length
The word count difference between the raw summary and the reference summary supports the value and quality of the summary writing task in Step 2, indicating that the raw summary still contains some redundant information. 

%% The compression rate
%The average input-summary length is 1055.6 and 114.8, which is \tingyao{longer than both CNN/DM (784.4 and 55.2), EmailSum (233.2 and 68.5) dataset, confirming the multiple QAs input to our task required summarization}. \todo{compare against other summarization datasets. Answer Summarization and EmailSumm, for example?}\yoshi{Not sure if we want to emphasize this. If not, let's remove}


%Detailed information is shown in \Cref{tab:ori-qa_dataset-stats}. 


% \begin{itemize}
% % Explain that we used the Amazon QA dataset\todo{CITE} and selected \todo{NUM} categories.

% \item Basic statistics of the dataset
% \end{itemize}


% Basic stats of the original dataset. For example,
% \begin{itemize}
%   \setlength{\parskip}{0cm}
%   \setlength{\itemsep}{0cm}
%   \item \# of product categories. 
%   \item \# of products.
%   \item Avg. \# of questions.
%   \item Avg. \# of answers.
% \end{itemize}

\iffalse

\subsection{Our Corpus}

We do statistic analysis on original dataset. We found, in each categories, most of the products contain at least 8 questions (better description?) and the product contains more answers per question if it contains more questions. We first remove the questions that length are short than 5 and longer than 15 for each product, because the shorter ones do not provide sufficient useful information and longer ones contain trivial contents without focusing on the information of the product. Then we filtered out the products that contain less than 8 unique questions. After merge duplicate items, our corpus contains 1777 items and 14,216 QA pairs in total. 


\todo{we should report the full list in Appendix) Probably, with some justification of why we chose the product categories.}


\subsection{Multi-stage Annotation}
The original Amazon QA dataset contains 5.94 questions and 23.29 QA pairs for each product on average. Since it is infeasible to ask the human annotator to write a summary from hundreds of QA pairs for each product, we designed a multi-stage annotation framework, which consists of three annotation steps, to create a high-quality QA summarization benchmark.

Figure~\ref{fig:annotation} depicts the schematic procedure of the multi-stage annotation framework.


\noindent
{\bf Step 1: QA-pair Rewriting} % (The first re-writing task)
First, we selected 8 unique QA pairs for each product (1777 products in total) and asked crowdsourced workers to rewrite each QA pair into declarative sentence(s). For each product, we used aggressive filter that follows the rules, (1) the tokens length of the questions should not small than 5 or more than 150, (2) neither the question nor the answer should contain first person pronouns, and (3) each question should be unique, to select representative QA pairs to cover the information described in the most of QA pairs for each product. Thus, we can assume that the content in the remaining QA pairs are substantially covered by the selected QA pairs. After selecting the representative 8 QA pairs, we recruit three crowd workers from Amazon Mechanical Turk to rewrite the 8 QA pairs for each item. The overview of designed interface is in Figure~\ref{fig:rewrite}. The rewriting annotation task can separate into three steps. (1) We first provide the product link on Amazon for the workers to help them have better understand of the product. (2) Then we set up certain rubrics as follow. 1. All the rewriting should be in declarative formats. 2. Keep all the useful information as much as possible even if the information is not answer the question straightforward. 3. Do not included your personal experience and use first person pronouns in the rewriting. 4. Try to summarize both question and answer information. 5. Do not use Yes/No in your answer. 6. If you describe the product, use "This product" or "This item" instead of "it" or "that". 7. Do not add extra information not included in question and answer, even though you found it on the product website. And we further provide concrete examples to let workers follow with the rewriting rules. (3) Finally, we show the 8 representative QA pairs in separate question and ask them to write a short summary. We also provide some warnings and rubrics along with each question to remind workers to follow the rules. We collect three assignments for each product and use error detection followed by our designed rubrics. Our error detection has several checks, Longest common subsequence (LCS), Yes/No, QA format, It/it, First person pronouns and Ignore Question info. We also use different weight to do error evaluation to choose the best one as our final rewriting QA pairs. 


\noindent
{\bf Step 2: Summary Writing} % (The second summary writing task)
We manually checked collected declarative sentences and observed that the sentences contained redundant/irrelevant information and have some minor grammatical issues. Thus, the simple concatenation of the collected sentences would not ensure the enough quality as a QA summarization benchmark. 
%
To address these issues and improve the fluency of the gold-standard summary, we published the second annotation task that asked crowdsourced workers to write summaries from the collected declarative sentences. 
%
\xiaolan{<Followed by the details of the task>} With this annotation step, now we have high-quality gold-standard summary for each product. 


\noindent
{\bf Step 3: Input QA-pair Enrichment} % (The sentence-pair "entailment" judgement task)
As described in Step 1, we selected representative QA pairs to make the summary creation step feasible. However, in practice, a product may have more than 8 QA pairs, and the benchmark with only 8 QA pairs may not represent the real-world scenario.
%
To make the benchmark more realistic, we use two data augmentation strategies. (1) We add the multiple QA pairs if the question is been selected as 8 representative questions. (2)We added QA pairs that can be ``entailed'' by the gold-standard summary for each product. Specifically, we first use sentence similarity (BERT sentence embedding) sampled QA pairs from the remaining QA pairs that were not used in the first re-writing task and then asked the crowdsourced worker to judge if a QA pair can be ``entailed'' by the gold-standard summary. We finally collect \xiaolan{number} QA pairs in total from the entailed task. By doing so, we can appropriately augment the input QA pair while keeping the gold-standard summary stay the same. After the data augmentation step, we remove those QA summaries that copies to much from the original QA pairs and filter out the product contains low quality QA summarizes. There are 1440 products and 39,485 QA pairs in our final dataset. Detailed information is shown in \Cref{tab:qa_dataset-stats}.



\fi

==> EMNLP-2022 CoQASum/sections/evaluation.tex <==
\begin{table*}[t]
%\small
    \centering
    \begin{tabular}{l|rrrr|ccc}
    \toprule  
    & \multicolumn{4}{c|}{\textbf{Performance}} & \multicolumn{3}{c}{\textbf{Supervision}} \\
     &\multicolumn{1}{c}{R1} &  \multicolumn{1}{c}{R2} &  \multicolumn{1}{c}{RL} &  \multicolumn{1}{c|}{BertS} & SeedQA & Rewr. QA & Gold Sum. \\ \midrule
    \textit{Extractive:} & &&&&\\
     \quad SeedQAs & 18.96 & 10.22 & 12.57 & 83.26 & - & - & -\\
     \quad LexRank & 33.17 & 9.30 & 19.26 & 83.76 & - & - & - \\
     %& LexRankBERT & 35.34 & 10.15 & 19.66 & 84.25 \\
     \quad BertSumExt & 31.81 & 11.10 & 19.38 & 84.57 & No & No & Yes \\ \midrule
     \textit{Extractive-Abstractive:}& &&&&\\
    \quad LexRank+LED & 35.92 & 8.97 & 18.37 & 84.37 & No & Yes & No\\
     %& LexRankBERT+LED & 36.35 & 8.74 & 17.84 & 84.45 \\
    \quad LED+LexRank & 38.01 & 10.71 & 19.98 & 84.01 & No & Yes & No\\
     %& LED+LexRankBERT & 36.99 & 8.94 & 17.80 & 84.19 \\
     %& LED+BertSumExt & 35.49 & 9.63 & 18.07 & 83.72 \\
    \quad BERT-SingPairMix & 40.82 & 12.73 & 21.28 & 85.17 & No & No & Yes \\
    \quad FastAbstractiveSum & 42.51 & 15.21 & 22.53 & 84.47 & No & No & Yes\\ \midrule

    % & PEGASUS & 44.02 & 49.80 & 45.28 & 17.31 & 20.00 & 18.00 & 23.93 & 27.52 & 24.81 & 24.80 & 26.03 & 25.47 \\
    
    % & T5 & 45.15 & 46.97 & 44.56 & 17.61 & 18.77 & 17.62 & 24.77 & 26.10 & 24.61 & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} \\
    
    % & BART & 48.10 & 51.48 & 48.19 & 20.85 & 22.77 & 21.13 & 26.72 & 28.87 & 26.89 & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} \\
    \textit{Abstractive:} & &&&&\\
    \quad LED & 45.82 & 19.34 & 26.01 & 87.55  & No & No & Yes \\
    % I rerun the checkpoint and the scores are higher when length increase, updated on Github repo.
    \quad  HierLED
    %Hier. LED
    %(HMNET)
    & 48.30 & 23.29 & 29.84 & 88.55 & No & No & Yes\\ 
    \quad \textbf{DedupLED} & \textbf{52.73} & \textbf{27.24} & \textbf{31.68} & \textbf{88.96} & Yes & No & Yes\\
     \bottomrule
    \end{tabular}
    \caption{
    %Performance of the task. We show the data that we used for supervison of each model. R1/R2/RL correspond to ROUGE1/2/L F1 scores and BS corresponds to BERTScore F1. With auxiliary objective, supervised by the selection of SeedQAs, DedupLED outperforms all the other alternatives.
    Performance of the models on \corpus{} and the type of supervision that each method used. R1/R2/RL/BS denotes ROUGE-1/2/L F1 and BERTScore F1, respectively. With the auxiliary objective, \model{} outperforms all the other alternative models.}
    \label{tab:result-summarization}
\end{table*}


%In this section, we show the experimental results based on three different methods we apply for our QA dataset. We randomly split the data into train/val/test sets, and have 1152/144/144 entities respectively. For LexRank, we limit the output length based on the average reference summary length in the training set. For LED and its variations, we fine-tuned the \texttt{allenai/led-base-16384} checkpoints from Hugging Face\footnote{\url{https://huggingface.co/}}. For all supervised methods, we report the performance of the best epoch, selected based on the validation set. 
We conduct comparative experiments to evaluate those models for the \task{} task on the \corpus{} dataset.
%
We randomly split the data into train/validation/test sets, which consist of 1152/144/144 entities, respectively. 
%
For LexRank, we limit the output length based on the average reference summary length in the training set. For LED and its variations, we fine-tuned the \texttt{allenai/led-base-16384} checkpoint using the Hugging Face Transformers library.~\footnote{\url{https://github.com/huggingface/transformers}} We report the performance of the best epoch (based on ROUGE-1 F1) chosen on the validation set for all the supervised models. 


%We provide detailed experiment setting of each model in the Appendix~\ref{sec:appendix:model-details}. \tingyao{feel like no in general common setting}



% put details in the appendix

% For all the end-to-end models, captions are decoded using the beam sampling strategy with beam size = ?, minimal length = ?, and maximum length = ?.
% For the FastAbstractiveSum, we pretrained the word2vec on our data for 200 epochs. We set the vocab size to 4000. Both extractor and abstractor train with batch size = 32. For the abstractor, we set up the maximum input length of each QA pair = 150, and output summary = 30. For the extractor, the maximum input length of each QA pair = 150 and maximum QA pairs = 30. Each summary are decoded using beam size = 5, maximum length = 30 and we concatenate them as final summary of each entity. For the abstractive methods, summaries are decoded using the beam sampling strategy with beam size = ?, vocab size =?

%\yoshi{Add explanations on experimental settings, including train/dev/test split. Especially, how product categories are split. Hyper-parameter tuning strategy etc.}

%The overall performance is shown in \Cref{tab:result-summarization}. We complete both automatic evaluation and human evaluation to do detailed comparision and analysis.

%\subsection{Auto Metrics}
\subsection{Automatic Evaluation}
%\yoshi{Comment: for summarization papers, we can simply say we use ROUGE-1/2/L and BERTScore with minimal additional information (if any).}
For automatic evaluation, we use ROUGE~\cite{lin2004rouge} F1\footnote{\url{https://pypi.org/project/py-rouge/}} and BERTScore~\cite{zhang2019bertscore} F1\footnote{\url{https://github.com/Tiiiger/bert_score}} with the default configuration. 
%For BERTScore, we used \todo{base model or simply say default configuration}
The performance and required supervision of all models described in Section~\ref{sec:models} are shown in Table~\ref{tab:result-summarization}. 



\iffalse
We evaluate the model performance using existed common auto-metrics methods, ROUGE and BERTScore, for summarization tasks.

\textbf{ROUGE} \cite{lin2004rouge} is a recall-based automatic evaluation method that has been widely used in summarization and machine translation task. ROUGE-N calculates the number of overlapping "n-grams" (n-words) between "generated text" and a gold "reference". N represents the number of consecutive words. We report (1) ROUGE-1 (R1) refers to unigram (each word) overlap between the generated and reference summaries. (2) ROUGE-2 (R2) refers to bigram overlap between the generated and reference summaries. (3) ROUGE-L (RL) calculates the longest common subsequence (LCS). We use \tingyao{add package link} and report the scores in \Cref{tab:result-summarization}.

\textbf{BERTScore} \cite{zhang2019bertscore} is a common evaluation method in recent generation task. It takes advantage of large pre-trained contextual embeddings from BERT\cite{devlin2018bert} and calculate the semantic similarity between candidate and reference summaries. We use \tingyao{add package link} and report precision, recall, and F1 measure scores.
\fi


\paragraph{Extractive:}% methods}
SeedQAs, which simply selects the original QA pairs, performs badly. This is expected because while with high recall ($88.45$ R1-recall), the Oracle method suffers badly from low precision, largely due to the sentence-type inconsistency (i.e., interrogative vs. declarative) and duplication in input QA pairs. 
%
LexRank, the unsupervised summarization baseline, performs slightly better than SeedQAs thanks to its ability to select more concise QAs for the output summary. BertSumExt, while leveraging gold-standard summaries, achieves similar performance with LexRank. We believe the discrepancy between interrogative and declarative sentences in input QA pairs and gold-standard summaries is the primary cause of the performance. 
%As shown, the Oracle method, which consists of the seed QAs we selected for annotation, performs badly. This is expected because while with high recall ($88.45$ R1-recall), the Oracle method suffers badly from low precision, largely due to the writing style and duplication between questions and answers. Lexrank, the unsupervised summarization baseline, performs slightly better than Oracle thanks to their ability to select more concise QAs in the summary. BertSumExt, despite leveraging the supervision from gold-standard summaries, achieves similar performance with LexRank. We believe the discrepancy between QA style and declarative style is the major cause of its current performance. 

%\textit{Takeaway: performance of the extractive methods confirms that sentence-type transfer from QA to declarative sentences is crucial for the \task\ task.}


%\yoshi{I'm here}

\paragraph{Extractive-Abstractive:}% methods}
Extractive-abstractive models achieve better performance than extractive models. The sentence-type transfer helps LexRank+LED/LED+LexRank achieve a much higher R1 score while comparative R2/RL/BS scores against the original LexRank. This implies the limitation of sentence selection before/after sentence-type transfer. Also, the sentence-type transfer model was trained on seed QA pairs and their corresponding declarative sentences, not the gold-standard summaries. Thus, another factor may be the difference between the rewritten QA pairs and the gold-standard summaries. 

Both FastAbstractiveSum and BERT-SingPairMix, which are directly supervised by the gold-standard summaries, show significantly better performance than the extractive models.
%
The results confirm that those models can learn to perform both sentence-style transfer and duplication removal directly from gold-standard summaries.
%Extractive-abstractive methods achieve better performance than extractive methods. In particular, the supervision from rewritten QA helps LexRank+LED and LED+LexRank to achieve much higher R1 score and comparative R2/RL/BS scores compared to LexRank.  Besides, both FastAbstractiveSum and BERT-SingPairMix, which are directly  supervised by the gold-standard summaries, show even better performance. This is also expected because the models can learn to perform both sentence-style transfer and duplication removal directly from gold-standard summaries.

%\textit{Takeaway: additional supervision for sentence-style transfer and duplication removal helps models achieve better performance.}

\paragraph{Abstractive:} All three models achieve strong performance on the \task\ task. The vanilla LED outperforms extractive/extractive-abstractive models. 
%
By incorporating the hierarchical structure into the model, HierLED improves the performance against the vanilla LED.
%
Furthermore, \model{} achieves the best performance for all the evaluation metrics. This confirms that by adding an auxiliary objective and using another supervision (i.e., seed QA pair selection), \model{} appropriately learns to deduplicate while learning to summarize input QA pairs. 

%All three models achieve strong performance on the \task\ task. In particular, DedupLED shows the best performance because of the auxiliary objective for duplication removal.

%\textit{Takeaway: from our experiment, we confirm that both sentence-style transfer and duplication removal are crucial for the \task\ task. In addition, pre-trained language model checkpoints can significantly improve the model performance. Finally, DedupLED, a multi-task variation of pre-trained LM, is a strong baseline for the \task\ task.}
\noindent {\bf Takeaway:}
\textit{From the results, we confirm that both sentence-style transfer and duplication removal are crucial for the \task\ task. In addition, fine-tuning pre-trained language models using the gold-standard summaries offers strong performance, better than manually-crafted two-stage summarization models. Finally, by incorporating the duplication removal functionality into the model via multi-task learning, we show that \model{} establishes a strong baseline for the \task\ task.}

%\Cref{tab:result-summarization}provide an overview of the evaluation results for three methods used on various models. The original eight QA pairs perform poorly, demonstrating the gap between original QA and summarizes. LexrankBERT outperforms all other extractive methods, including BertSumExt, a deep extractive method. However, BertSumExt perform the best in BERTScore vice versa. Compared to purely extractive methods, extractive-abstractive methods improve performance even more. FastAbstractiveSum outperforms pretrained model combing methods when using RL with hybrid models. The large-scale pretrained models provided a solid foundation for our CQA tasks. The fully-supervised strategy perform the best among three methods. LED takes advantage of huge pretrained knowledge and demonstrates the ability to adapt specific task by fine-tuning. We compared three different strategies based on LED model. HierarchicalLED has better performance than non-hierarchical baseline, however it is not the best option. It is not surprising that DedupLED perform the best among the end-to-end models. \tingyao{core idea of DedupLED}. 

% condense a large number of QA pairs into a concise and declarative format.
%\tingyao{(1) final the table. (2) naive vs multi-task vs hier. (3) other take away}


\subsection{Human evaluation}
We further conducted human evaluation to judge the quality of generated summaries by different models.
%
For every entity in the test set, we showed summaries generated by four models (LexRank, FastAbstractiveSum, BERT-SinglePairMix, and DedupLED) to three human judges\footnote{\url{https://appen.com/}} to choose the \textit{best} and \textit{worst} summaries for three criteria: informativeness (Inf.), coherence (Coh.), and conciseness (Con.). Then, we computed the performance of the models using the Best-Worst Scaling~\cite{louviere2015best}.
%
Table~\ref{tab:human_eval} shows that \model{} consistently achieves the best performance in all three criteria. On the other hand, LexRank, as expected, performs the worst among all the methods we tested.
%
The human evaluation performance trend aligns with the automatic evaluation performance, validating the quality of \corpus\ as a benchmark for the \task\ task.

%We further conducted human evaluation to judge the quality of generated summaries. For every entity in the test set, we asked three human judges to indicate the \textit{best} and \textit{worst} summary according to three criteria: informativeness (Inf.), coherency (Coh.), and conciseness (Con.). We further compute the performance of different models using Best-Worst Scaling~\cite{louviere2015best}. As shown in Table~\ref{tab:human_eval}, DedupLED achieves better performance than the alternative methods in all three dimensions. Meanwhile, LexRank, as expected, behaves the worst among all methods we tested. Besides, the human evaluation performance also aligns with the automatic evaluation performance, indicating that our \corpus\ benchmark can effectively evaluate the \task\ task.
%We further do human evaluation to investigate the performance if the auto mertrics evaluation is correlated to human judgement. \tingyao{say something according to result}

\begin{table}[]
\small
    \centering
    \begin{tabular}{l|c|c|c}
    \toprule
    & Inf. & Coh. & Con. \\ \midrule
    LexRank &-8.41&-5.72&-8.42 \\
    FastAbstractiveSum &-4.71&+1.01&+3.37 \\
    BERT-SingPairMix &-2.02&-6.07&-1.35 \\
    DedupLED &+13.13&+5.72&+4.38\\\bottomrule
    \end{tabular}
    \caption{Best-Worst Scaling on human evaluation.}
    \label{tab:human_eval}
\end{table}

\begin{comment}
\begin{table*}[t]
    \tiny
    \centering
    \begin{tabular}{llrrrrrrrrrlll}
    \toprule \hline
    Methods & \multicolumn{1}{c}{Models} & \multicolumn{1}{c}{R1-P} & \multicolumn{1}{c}{R1-R} & \multicolumn{1}{c}{R1-F} & \multicolumn{1}{c}{R2-P} & \multicolumn{1}{c}{R2-R} & \multicolumn{1}{c}{R2-F} & \multicolumn{1}{c}{RL-P} & \multicolumn{1}{c}{RL-R} & \multicolumn{1}{c}{RL-F} & \multicolumn{1}{c}{BERT-P} & \multicolumn{1}{c}{BERT-R} & \multicolumn{1}{c}{BERT-F} \\ \hline
    \multirow{4}{*}{Extractive} & Original 8 QAs & 10.85 & 88.45 & 18.96 & 5.81 & 49.51 & 10.22 & 7.17 & 60.13 & 12.57 & 86.25 & 80.49 & 83.26 \\
     & LexRank & 31.47 & 37.98 & 33.17 & 8.79 & 10.64 & 9.30 & 18.09 & 22.31 & 19.26 & 83.09 & 84.51 & 83.76 \\
     & LexRankBERT & 33.45 & 40.28 & 35.34 & 9.55 & 11.57 & 10.15 & 18.43 & 22.64 & 19.66 & 83.57 & 85.00 & 84.25 \\
     & BertSumExt & 49.66 & 24.98 & 31.81 & 17.29 & 8.68 & 11.10 & 30.32 & 15.17 & 19.38 & 84.91 & 84.28 & 84.57 \\ \hline
    \multirow{7}{*}{2-stage} & LexRank+LED & 35.42 & 39.89 & 35.92 & 8.85 & 9.92 & 8.97 & 18.03 & 20.52 & 18.37 & 83.99 & 84.79 & 84.37 \\
     & LexRankBERT+LED & 35.10 & 40.97 & 36.35 & 8.44 & 9.74 & 8.74 & 17.20 & 20.14 & 17.84 & 83.80 & 85.15 & 84.45 \\
     & LED+LexRank & 35.46 & 44.16 & 38.01 & 9.79 & 12.66 & 10.71 & 18.49 & 23.44 & 19.98 & 82.92 & 85.22 & 84.01 \\
     & LED+LexRankBERT & 33.68 & 44.47 & 36.99 & 8.15 & 10.63 & 8.94 & 16.13 & 21.48 & 17.80 & 82.97 & 85.52 & 84.19 \\
     & LED+BertSumExt & 39.75 & 34.66 & 35.49 & 10.90 & 9.29 & 9.63 & 20.31 & 17.57 & 18.07 & 82.70 & 84.81 & 83.72 \\
     & FastAbstractiveSum & 44.89 & 44.27 & 42.51 & 15.84 & 16 & 15.21 & 23.7 & 23.62 & 22.53 & 83.77 & 85.21 & 84.47 \\
     & BERT-SingPairMix & 49.96 & 37.55 & 40.82 & 15.36 & 11.83 & 12.73 & 26.21 & 19.54 & 21.28 & 85.41 & 84.95 & 85.17 \\ \hline
    \multirow{6}{*}{end-to-end} & PEGASUS & 44.02 & 49.80 & 45.28 & 17.31 & 20.00 & 18.00 & 23.93 & 27.52 & 24.81 & 24.80 & 26.03 & 25.47 \\
     & T5 & 45.15 & 46.97 & 44.56 & 17.61 & 18.77 & 17.62 & 24.77 & 26.10 & 24.61 & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} \\
     & BART & 48.10 & 51.48 & 48.19 & 20.85 & 22.77 & 21.13 & 26.72 & 28.87 & 26.89 & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} \\
     & LED & 46.93 & 47.74 & 45.82 & 19.58 & 20.34 & 19.34 & 26.48 & 27.27 & 26.01 & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} \\
     & LED multi-task & 52.10 & 52.31 & 50.80 & 25.35 & 25.92 & 24.99 & 30.71 & 31.16 & 30.12 & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} \\
     & Hier. LED (HMNET) & 51.33 & 49.46 & 48.91 & 23.19 & 23.48 & 22.53 & 29.97 & 30.14 & 29.26 & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} \\ 
     \hline \bottomrule
    \end{tabular}
    \caption{Summarization Result\todo{finalize table, F1-scores, remove others pretrained models results}}
    \label{tab:result-summarization}
\end{table*}

\end{comment}


==> EMNLP-2022 CoQASum/sections/introduction.tex <==
\begin{figure}[t]
\includegraphics[width=0.49\textwidth]{fig/example-3.pdf}
    \caption{Example of the \task\ task. The input contains a collection of QA pairs. Duplicated information can be found in a single QA pair or across multiple QA pairs. The output is a concise and coherent summary written in declarative sentences.  }
    %\yoshi{Highlighting corresponding part may be helpful.}\yoshi{This figures does not explicitly show ``duplicate'' questions/answers. It may be difficult to show everything in one figure, though.}\tingyao{make update and edit file}}
    \label{fig:amazon_qa}
\label{fig:example}
\end{figure}
% Figure link: https://docs.google.com/drawings/d/1MDoUwrOnHs-aU6p-Y6lmJlDcf9VzqbC1YM5yU-imcls/edit?usp=sharing
% Figure link: https://docs.google.com/drawings/d/180LebQoHa57ZMPs2j65dVKGiRbPO4YCdlIZpbS410UE/edit

%% CQA is important
Community-based Question Answering (CQA) enables users to post their questions and obtain answers from other users. With the increase in online services, CQA has become essential for various purposes, including online shopping, hotel/restaurant booking, and job searching. Many online platforms implement CQA features to help users acquire additional information about entities (e.g., products, hotels, restaurants, and companies) of their interests.
%
CQA complements customer reviews---another type of user-generated content, which provide additional information about the entity but mostly focusing on user experiences and their opinions. %\yoshi{Explicitly adding CQA provides more factual information? Need backup evidence, though}
%complements ``question-agnostic'' customer reviews, providing additional information not described in the official entity description (e.g., product descriptions,  general information of hotels/restaurants).\yoshi{Customer reviews tend to summarize customer experiences while CQA more focus on factual information. This is one way to differentiate from the line of opinion summarization research.}

%% What is still missing?
While CQA greatly benefits users in decision-making, digesting information from original question and answer pairs (QA pairs\footnote{In this paper, we use QA pairs to refer to question-answer pairs in CQA.}) also has become increasingly harder. %\yoshi{Todo: word choice}
%
Due to the community-based nature, CQA tends to have a large number of heavily repetitive QA pairs, %, which contain highly repetitive questions/answers.\yoshi{Citation if possible}, 
which make it difficult for users, especially those who do not have specific intent (i.e., questions), to find and digest key information. 

Existing summarization efforts for CQA~\cite{liu2008understanding,Deng:2020:AAAI,AnswerSumm} primarily focus on summarizing answers for a given question, which still assumes that the user has a certain intent.
%
We believe that information spread over QA pairs can be summarized into a more concise text, which helps any users grasp the key points of discussions about a target entity.
%
Therefore, we take a step beyond the scope of answer summarization and propose a novel task of \task, which aims to summarize a collection of QA pairs about a single entity into a concise summary in declarative sentences (shown in Figure~\ref{fig:amazon_qa}).


%% We propose a novel task
% \yoshi{TODO: Revise this paragraph, referring to the line of Answer Summarization and its limitations}
% We believe that key information spread over CQA can be converted into a more concise summary, which helps any type of user grasp the point of conversations about a target entity. To address this issue, we propose the task of \task, which aims to summarize a collection of QAs about a single entity into a concise summary written in declarative sentences (shown in Figure~\ref{fig:amazon_qa}).
%
% Input format is different
% \task{} considers a collection of questions and their answers as input, unlike existing Question Answering summarization efforts~\cite{see-etal-2017-get, liu2008understanding, deng2020joint, fabbri2021answersumm}, which primarily focus on summarizing answers for a given question. \yoshi{We should defend a potential criticism on ``Why don't you guys apply this method first and then aggregate summaries into one?''}\tingyao{We believe that the questions play an important role in addressing the lack of key information in the answers. (not sure if it's sufficient)} We will show that both questions and answers contain essential information, so we cannot simply use one to make a summary. \tingyao{maybe put an example?}

%% Challenges in CQA summarization
The \task{} task has the following two unique challenges.
%
% 1) Sentence-type/writing-style transfer
First, \task{} needs to solve sentence-type transfer %\yoshi{term needs to be defined. Writing-style transfer may not be accurate}
as questions in interrogative sentences have to be converted into declarative sentences to make a concise summary. This challenge is not trivial as existing summarization tasks assume that input and output are both written in declarative sentences. 
%
% 2) Duplicates?
Second, CQA contains duplicated questions and answers. That is, different users can post similar questions. A question can have multiple answers, many of which contain duplicate information. % but sometimes contain very specific and unique information. This makes it difficult to simply remove duplicate questions and answers from CQA.
%
Also, unlike question-answering forums (e.g., Quora), CQA in online services is less incentivized to remove such redundancy. Slightly different questions/answers can provide detailed and useful information not mentioned in other questions/answers. Having more similar answers supports the information is more reliable.% \yoshi{Somebody may mention the voting function in CQA.}
%
Those properties make existing summarization solutions unsuitable for \task. 

To enable further study of the \task\ task, we create a corpus \corpus{} by collecting reference summaries on QA pairs from the Amazon QA dataset \cite{wan2016modeling, mcauley2016addressing}.
%
Reference summary annotation is challenging for \task, as a single entity (i.e., a product for the dataset) can have so many questions and answers that the annotator cannot write a summary directly from them. Furthermore, the sentence-type difference (i.e., interrogative vs. declarative) obstructs summary writing. 
%
To make this annotation feasible, we designed a multi-stage annotation framework. Sampled seed QA pairs are given to the annotator to convert into declarative sentences, which are then rewritten into gold-standard summaries by expert writers. At the last step, we collected semantically similar QA pairs to to make the annotated corpus more realistic. 


%% Our solution
We conduct a comprehensive experiment that compares a collection of extractive and abstractive summarization solutions and establish a strong baseline approach, DedupLED, for the \task\ task. Specifically, \model{} fine-tunes the entire LED model for summary generation while additional classifier attached to the encoder is optimized to extract representative QA pairs. Leveraging the strengths of both abstractive and extractive summarization objectives, as well as the pre-trained language model checkpoints, DedupLED significantly outperforms the other alternative methods. 
Our experiment also confirms that \model{} is suitable for \task, as the model implements the functionality for both (1) sentence-type transfer and (2) duplicate removal.

%To this end, we develop a multi-task CQA summarization model \model, which leverages the strengths of both abstractive and extractive summarization models. Specifically, \model{} fine-tunes the entire LED model for summary generation while additional classifier attached to the encoder is optimized to extract representative QA pairs. 
%
%This design makes \model{} suitable for \task, as the model should implement the functionality for (1) sentence-type transfer and (2) duplicate removal.
%
% For (1), we consider fine-tuning a pre-trained Transformer encoder-decoder model on training data, expecting that the model learns to rewrite and summarize input QA pairs in an end-to-end manner.
% %
% For (2), we add another classifier layer that is optimized for extractive summarization to facilitate the model further to exclude duplicate information. 
% % We found that simply fine-tuning a model on training data is insufficient for the task.


%% Corpus creation
%To establish an evaluation benchmark for \task, 
%For evaluation, we create a corpus \corpus{} by collecting reference summaries on QA pairs from the Amazon QA dataset \cite{wan2016modeling, mcauley2016addressing}.
%
%Reference summary annotation is challenging for \task, as a single entity (i.e., a product for the dataset) can have so many questions and answers that the annotator cannot write a summary directly from them. Furthermore, the sentence-type difference (i.e., interrogative vs. declarative) obstructs summary writing. 
%
%To make this annotation feasible, we designed a multi-stage annotation framework. Sampled QA pairs are given to the annotator to convert into declarative sentences, which are then rewritten into summaries by expert writers. At the last step, we collected semantically similar QA pairs to enhance the annotated corpus to make the corpus more realistic. 

 

%% Experimental results
%We conduct a comprehensive experiment that compares a variety of existing summarization solutions and \model{} on \corpus.
%
%Experimental results confirm that \model{} significantly outperforms other baselines, confirming that the two characteristics are essential to solving \task. Because extractive methods do not compare with abstractive solutions, we further confirm that addressing both (1) sentence-type transfer and (2) duplication removal is not trivial for solving our task. \tingyao{change last sentence a bit}

% Also, observing existing extractive summarization models do not match against abstractive solutions, we confirm that addressing both (1) sentence-type transfer and (2) duplication removal are not trivial for the existing solutions. \yoshi{The last sentence is awkward.}

%essential for the task. \yoshi{Just dumping potential claims here, which may not be supported. Feel free to edit directly.}

%% Our contributions
Our contributions of the paper are as follows:
\begin{itemize}
    \setlength{\parskip}{0cm}
    \setlength{\itemsep}{0cm}
    \item We propose the novel task of \task, which takes QA pairs about a single entity as input and make a summary written in declarative sentences (Section~\ref{sec:problem}). 
    \item We designed a multi-stage annotation framework and collected reference summaries to build the first benchmark corpus for \task. The corpus is based on the Amazon QA corpus~\cite{wan2016modeling} and consists of reference summaries for $1,440$ entities with $39,485$ QA pairs from 17
    %\todo{check}\tingyao{correct}
    product categories. (Section~\ref{sec:corpus}). 
    \item We conduct comprehensive experiments on a collection of extractative and abstractive summarization methods and develop a strong baseline \model, which implements key characteristics of sentence-type transfer and duplication removal functions. %Through comprehensive experiments that also tested a series of extractive and abstractive summarization models, we show that \model{} establishes a strong baseline for \task. 
    (Section~\ref{sec:models} and Section~\ref{sec:evaluation}). 
\end{itemize}



==> EMNLP-2022 CoQASum/sections/introduction_old.tex <==
\begin{figure}[t]
\includegraphics[width=0.49\textwidth]{fig/example.pdf}
    \caption{Example of the \task\ task.}
    \label{fig:amazon_qa}
\label{fig:example}
\end{figure}
% Figure link: https://docs.google.com/drawings/d/1MDoUwrOnHs-aU6p-Y6lmJlDcf9VzqbC1YM5yU-imcls/edit?usp=sharing

%Besides reviews, many e-service such as Amazon, Indeed, etc. websites now provide Questions and Answers (Q\&A) functionality for users to post their questions and also provide answers for others. (See the provided examples in \Cref{fig:indeed_qa}, \Cref{fig:amazon_qa}). Thus, Q\&A becomes an important resource for people to acquire the desired information. Meanwhile, the number of Q\&A pairs is consistently growing, which makes it hard for users to quickly digest information mentioned in existing Q\&As. Although most e-service consists of various items with question-answering data and reviews, we found there are some common properties between. (1) Most of product contains multiple questions and answers; (2) Many questions are repetitive and sometimes are either too short or too long that is unclear what the customers want to ask; (3) Answers are quite different from customers if it is an open questions because people tend to answer based on their experience or preference. Base on above properties, it becomes harder for the users to obtain useful and concrete information in just a couple of minutes. 

%\hl{

E-commerce platforms have became an essential component in our daily life. People nowadays use such platforms to perform a variety of tasks from online shopping, hotel/restaurant booking, to even job searching. Most of them use Community Question Answering (CQA) to help user acquire additional information about an entity (e.g., a product or a hotel). \kenneth{The paper didn't explain what is an ``entity''. You kinda need to clarify it, as in NLP an ``entity'' means something quite specific.}, such as the serving time of the breakfast in a hotel or the warranty of a product.\kenneth{I would use a different example. Since you want to emphasize ``extra'' information, I'd use some information that is obviously NOT in the manual.}
While such information can greatly benefit users in the decision making process, accessing the information mentioned in existing QAs is not always easy, especially when users do not know what to ask but still want to digest the important information the others mentioned.
This is because there often exits a large number of QAs with heavily repetitive questions and answers.
To address this issue, our goal is to summarize a collection of QAs from an entity (Figure~\ref{fig:example} (a)) into a concise and declaritive summary (Figure~\ref{fig:example} (b)), which we refer as the \textit{\task\ problem}.\kenneth{This is minor, BUT why not say it's ``CQA Summarization''? People know what CQA is.}

Unlike existing question and answering summarization works~\cite{see-etal-2017-get, liu2008understanding, deng2020joint}, which mainly focus on summarizing answers for one given question, the \task\ problem considers a collection of questions and their answers as the input.\kenneth{This is correct. So why did you decide to use the same name? ``QA Summarization'' has been used I think.}
Besides, the \task\ problem highlights two properties for a desired summary. First, like other summarization tasks, we want to exclude repetitive content by producing a \textit{concise} summary.
Second, instead of presenting a set of QAs, we want to generate a \textit{declarative} summary (i.e., summary in plain text) to further help readers quickly and easily digest the information.\kenneth{Now I see where does the word come from. BUT ``declarative'' is still quite confusing. I would use a more simple word.}
This property further makes existing opinion summarization solutions~\cite{meansum, suhara-etal-2020-opiniondigest}\todo{add more} unsuitable to solve the \task\ problem as they mainly takes plain text, i.e., reviews, as the input and rarely perform style transfer during the summarization process.

\kenneth{One argument missing here is why this is different from traditional summarization task. Because CQA data tends to be more repetitive?}

\kenneth{A higher-level argument (which may or may not be important) for CQA is that users with different needs can find what they want in the QAs. This paper kinda wants to say that users generally want to know the same set of information, which motivates the generation of summary. Not sure how important this is, but proably good to think about.}

A key challenge of the \task\ problem is the lack of training examples since none of the existing summarization benchmarks take a collection of questions and answers as the input and produce a declarative summary.
To address this challenge, we proposed a non-trivial data annotation process and created a benchmark dataset. With the benchmark dataset, we are then able to compare and study difference summarization models. Our contributions of the paper are as follows:
\begin{itemize}
    \item We propose a novel \task\ problem that takes multiple questions and answers from an entity as the input and generates a summary in the declarative form (i.e., plain text) (Section~\ref{sec:problem}). 
    \item We present a non-trivial data annotation framework to collect reference summaries and build the first benchmark dataset, which includes annotated summaries for $1440$ entities with $11.5K$ QA pairs, on Amazon CQA corpus~\cite{wan2016modeling}. Our annotation framework can also be applied for CQA corpus in other domains (Section~\ref{sec:corpus}). 
    \item We conduct a comprehensive empirical experiments for a series of extractive and abstractive summarization models and evaluated these models with both automatic and human evaluation. Through our experiments, we further establish strong baselines for the \task\ problem (Section~\ref{sec:models} and Section~\ref{sec:evaluation}). 
\end{itemize}

\kenneth{I don't think you need to have this outline for the paper for NLP papers. Can cut when need more space.}


%\todo{write a paragraph summarizing the key content and contribution of the paper.}\tingyao{I am done, feel free to modify this section}
\xiaolan{made a pass.}



%\begin{figure*}
%    \includegraphics[width=0.4\textwidth]{fig/indeed_qa.png}
%    \caption{Question \& Answering pairs for Dairy Queen at Indeed.com.}
%    \label{fig:indeed_qa}
%\end{figure*}

%\begin{figure*}
%    \includegraphics[width=0.4\textwidth]{fig/amazon_qa.png}
%    \caption{Question \& Answering pairs for "Conair HLM10 Hot Lather Machine" at Amazon.com.}
%    \label{fig:amazon_qa}
%\end{figure*}



%Existing summarization efforts on question and answering is mostly over a single question, i.e., how to summarize answers for a given question. \cite{see-etal-2017-get, liu2008understanding, deng2020joint} \todo{add for deng}. However, little work has been done over for summarizing all Q\&A postings for a given entity. \citet{suhara-etal-2020-opiniondigest} summarizes hundreds of user reviews, providing summaries for Q\&As is particularly helpful for users who want to digest information in Q\&A sessions but do not want to spend too much time browsing them, we take this advantage of our Q\&As summary. In addition, to make the summary concise, instead of presenting a set of selected Q\&As, we also want to summarize them in the declarative form, i.e., plain text. Thus, the core question we want to solve in this project is “how to summarize the most important, or most frequently asked questions in the Q\&A sessions?”. 
\iffalse

We introduce the QA summarization task as a result of the preceding intuition and existing limitation. Given a set of questions and answers, generate a declarative and informative summary. As far as we know, we are the first to propose the task. Our benchmark is built upon Amazon QA dataset, one of diverse and large-scale CQA dataset collected by \cite{wan2016modeling} from the product website. 
% xiaolan: I think we don't need to describe amazon QA dataset too much in the intro. Only highlight our dataset is enough. 
We first determined which items had lower quality QAs and obtained 1440 items and 11520 QA pairs in total. We then use human annotation in two steps to collect high-quality summaries. Finally, we use our dataset to establish strong baselines in three common summarization task approaches. 
% xiaolan: three common summarization approaches is not very clear. People may wonder "what three common approaches?" 
In general, we believe our proposed framework can be applied to any CQAs other than Amazon QA.
% xiaolan: sequence of the description is a bit twisted. I guess the framework here is about the annotation. So, in this paragraph, you first talked about problem -> annotation -> baselines -> annotation. Annotation appears twice. I believe it is better only mention it once.  



Overall, we claim the following contributions for our work.
\begin{itemize}
    \item We propose a new Amazon QA dataset as a high-quality resource for the QA summarization task.
    \item We conduct a thorough empirical model study and human evaluation analysis, which is critical for future research.
    \item Our framework is applicable not only to Amazon QA, but also to other domains of CQA dataset. 
\end{itemize}

Section \ref{sec:problem} defines our problem. Section \ref{sec:corpus} describes our framework for collecting the dataset. In Section \ref{sec:models}, we set up a comprehensive expriment and present both human and automatic evaluation in Section \ref{sec:evaluation}. In Section \ref{sec:analysis}, we conduct three different comparisons to analyze the experimental results.
\fi

==> EMNLP-2022 CoQASum/sections/models.tex <==
%To examine the feasibility and explore the challenges of our purprosed QA summarization task, we established several baselines and tested them using collected data described in the previous section. Our experiment separates into three categories, Extractive, Extractive-Abstractive and Abstractive methods. 
%\todo{put training details to Appendix?}
To examine the feasibility and explore the challenges of \task, we tested several summarization solutions on \corpus. The models are grouped into {\em Extractive}, {\em Extractive-Abstractive} and {\em Abstractive} methods. 

%\url{https://docs.google.com/document/d/1mLno5SRwlb3DiBQKQ7qwtffqSYJ-kWkLg9nw_DWF1oQ/edit}

%\yoshi{Say something like we develop a strong baseline on the task...?} \xiaolan{maybe in next section?}

\subsection{Extractive}
% Extractive methods tries to extract salient QAs as the summary. Under this category, we consider both unsupervised models, e.g., Lexrank~\cite{erkan2004lexrank}, and supervised models, e.g., BertSumExt~\cite{liu2019text}, for the \task\ task.
%
Extractive methods extract salient sentences from input QA pairs as the output summary. We consider unsupervised (LexRank) and supervised (BertSumExt) models in addition to a simple rule-based baseline that filters the original seed input QA. 
%
We evaluate those methods to understand how well selecting sentences without sentence-type transfer performs on the task.


%\paragraph{Oracle} The Oracle method simply concatenates the seed QAs we sampled from Sub-task 1 (Section~\ref{sec:annotation}). 
\paragraph{SeedQAs:} This method concatenates the seed QA pairs used in the first annotation task of the multi-stage annotation framework. This is an oracle method as we cannot tell which QA pairs were used as seed QA pairs for annotation. We use this method to verify the performance of simply extracting QA pairs. 

% We concatenate the 8 representative QAs that are selected for the first rewriting task of each item as summary.

% \paragraph{LexRank~\cite{erkan2004lexrank}} A common unsupervised extractive method for text summarization. It first uses degrees of similarity between words and phrases and computes the centrality of the sentences to build a graph. Then select the top-rank sentences as summary. 
\paragraph{LexRank~\cite{erkan2004lexrank}:} This is an unsupervised extractive method, which uses the similarity between words to build a sentence graph and compute the centrality of sentences for selecting top-ranked sentences as summary. 

%\textbf{Lexrank.} \cite{erkan2004lexrank} A common unsupervised extractive method for text summarization. It first uses degrees of similarity between words and phrases and computes the centrality of the sentences to build a graph. Then select the top-rank sentences as summary. 


%\textbf{LexrankBERT.} \xiaolan{}

% \paragraph{BertSumExt~\cite{liu2019text}} BertSumExt is a supervised approach which leverages BERT~\cite{devlin2019bert} to obtain the sentence representations and classify if a sentence should be included in the summary. In our experiment, we use BertSumExt to extract salient QAs from the input where the ``gold-standard'' labels are acquired using the greedy algorithm\footnote{\url{https://github.com/nlpyang/BertSum}}. 
\paragraph{BertSumExt~\cite{liu2019text}:} BertSumExt is a supervised model, which fine-tunes BERT~\cite{devlin2019bert} to extract sentences by solving multiple sentence-level classifications. 
%
In our experiment, we use BertSumExt to extract salient QA pairs from the input, where the gold-standard labels are acquired by greedily select QA pairs that maximize the ROUGE scores to the gold-standard summary\footnote{\url{https://github.com/nlpyang/BertSum}}.
%\yoshi{``The last sentence is unclear. How were the labels prepared?} \xiaolan{fixed}




\subsection{Extractive-Abstractive}
% While extractive methods can remove duplication from the input, they cannot transfer QAs into declarative sentences. To address this issue, we consider the extractive-abstractive methods, which not only extract salient QAs but also rewrite selected QAs in an abstractive manner. In particular, we consider both two-stages and end-to-end solutions for approach, which use the post-edited QA pairs from Sub-task 1 to train a separate sequence-to-sequence model to transfer the sentence-type. Besides, we also consider end-to-end models that learn to extract and rewrite QAs at the same time. 
While extractive methods can remove duplication from the input, they cannot transfer interrogative sentences (i.e., questions) into declarative sentences.
%
To handle this better, we combine extractive and abstractive models to implement two-stage solutions. We also test an existing two-stage algorithm in addition to another summarization model that learns to extract and rewrite in an end-to-end manner. 

%While extractive methods can help to remove duplication from the input, they can In this section, we use semi-supervised learning to extract the summary. We apply two-stage approach to combine extractive and abstractive methods. We first use abstractive method, then extractive method or vice versa to mimic semi-supervised approach. We also apply existing strong(?) semi-supervised models to extract the summary. 

\paragraph{LexRank+LED} 
% The post-edited QAs from Sub-task 1 (Section~\ref{sec:annotation}) allows us to train a sequence-to-sequence model that transfer individual QA into declarative sentences. Here we fine-tuned the LED model~\cite{beltagy2020longformer} to transfer the sentence-type of QAs. Essentially, after obtaining salient QAs from LexRank, we further feed them to the fine-tuned LED to obtain the declarative summary.
This method is a {\em select-then-rewrite} hybrid model. Using a sentence-type transfer model, the model rewrites each of the QA pairs extracted by LexRank into declarative sentences, which are then concatenated as an output summary. 
%
For the sentence-type transfer model, we fine-tune the LED model~\cite{beltagy2020longformer} on the seed QA pairs and their rewritten texts collected in Step 1 of the multi-stage annotation pipeline (Section~\ref{sec:annotation}). 

\paragraph{LED+LexRank} 
% This method reverse the steps of the above method. It first use the fine-tuned LED to convert all input QAs into declarative sentences, and then apply LexRank to form the summary.
This method is a {\em rewrite-then-select} hybrid model that swaps the steps of LexRank+LED. It uses LexRank to extract salient sentences from input QA pairs rewritten by the same sentence-type transfer model.

\paragraph{Bert-SingPairMix~\cite{lebanoff2019scoring}} Bert-SingPairMix is a select-then-rewrite-style model that first selects salient sentences from the input and then summarizes the selected sentences into the summary. In our experiment, we use our gold-standard summaries to train both the content selection model and the abstractive summarizer. %Bert-SingPairMix is a two-stages approach that first select salient sentences from the input and then compress information from the selected sentences into the summary. In our experiment, we use our gold-standard summaries to train both the content selection model and the abstractive summarizer. 
%\tingyao{In our experiment, we use rewritten summary to train both the BERT-based content selection model and the abstractive summarizer.}
%In our experiment, we use the seed QAs to train the BERT-based content selection model and the post-edited QAs to train the abstractive summarizer.  \todo{@Ting-yao: please confirm how the model was trained.}

%\textbf{BERT-SingPairMix.}Similar to extractive-abstractive method, \citet{lebanoff2019scoring} propose a model to compress or fuse the sentences from a single or pair representative sentences to generate a summary. The model consists of two parts, a sentence scoring model and a seq2seq sentence generation model. Again, we combine each question-answer pair as our as input.



\paragraph{FastAbstractiveSum~\cite{chen2018fast}}
FastAbstractiveSum also implements select-then-rewrite summarization via reinforcement learning. The model learns to select representative sentences with the extractor and rewrite the selected sentences with the abstractor. We train a FastAbstractiveSum model on the gold-standard summaries.
%FastAbstractiveSum is a end-to-end model that selects the representative sentences with an extractor and rewrites the selected sentences via an abstractor. Here we use FastAbstractiveSum to perform both the salient QA selection and the sentence-style transformation supervised by our gold-standard summaries. 
%\tingyao{We only use rewritten summary to supervised our model for all input QAs}. 
%Similar to the above approaches, we only use the post-edited seed QAs to train the model. \todo{@Ting-yao: please confirm how the model was trained.}

%Similar to extractive-abstractive method, use a hybrid model that first selects the representative sentences from each document and rewrites them into an abstractive format as a final summary. We adapt this model to our \task\ task. We concatenate each QA as one sentence unit. We pairs question-answer sentences with summary as input. We want the extracted model find the salient question-answer pair instead of question and answer separately. 



\subsection{Abstractive}
%Finally, we explore abstractive methods for the \task\ task. In particular, we fine-tuned pre-trained language models and their variations with our annotated \corpus\ benchmark dataset. 
As the final group of models, we explore abstractive models that directly summarize input QA pairs. Specifically, we use LED and its variants, which can take long-document as input. Our \model{} is a variant of LED and falls into this group. 


%In this section, we use fully supervised learning to extract the summary. We apply state-of-the-art pre-trained model and fine-tuned on our QA dataset in a end-to-end manner. We compare different fine-tuning methods to further investigate if it can improve our QA summaries quality. \\
% \textbf{PEGASUS.}

% \textbf{T5.}

% \textbf{BART.}

\paragraph{LED~\cite{beltagy2020longformer}} 
This model fine-tunes Longformer Encoder-Decoder (LED)~\cite{beltagy2020longformer} on input QA pairs and the gold-standard summaries in the training set. 
%To accommodate long sequences of the input QAs, we first consider fine-tuning Longformer~\cite{beltagy2020longformer} for the \task\ task. Note that LED is fine-tuned in a supervised manner where the input is the concatenated QAs and the output is the gold-standard summaries. 

%\textbf{LED.} Transformer-based models have successfully achieved state-of-the-art performance on a lot of NLP tasks including summarization task. It is usually suffered from  lack of processing long sequences. Longformer \cite{beltagy2020longformer} is one of them pretraining on huge English data, but deal with longer sequence such as language model. Due to the nature length of QA pairs in real-world scenario, we use Longformer-based model for comparison. We finetune Longformer on our Amazon QA dataset. Although the pretrained model did not train on QA format dataset, it show competitively results compared to both extractive and extractive-abstractive methods.

\paragraph{HierLED~\cite{zhu2020hierarchical,zhang2021emailsum}}
Hierarchical LED (HierLED) is a variant of LED, which has two encoders for token-level and QA-level inputs to handle the structure of QA pairs better. %\yoshi{Can you check if this description is correct?}\tingyao{that's correct} 
We use the same architecture as Hierarchical T5~\cite{zhang2021emailsum}, replacing T5 with LED. We fine-tune the model in the same manner as LED.
%Hierarchical LED utilizes the hierarchical structure to support long input sequences. In our experiment, we follow similar model architecture~\cite{zhang2021emailsum} but use Longformer~\cite{beltagy2020longformer} as backbone for the \task\ task. Again, the model is trained by the concatenated QAs and the gold-standard summaries. 

%\textbf{Hierarchical LED.} Hierarchical language models have been successfully perform well on several different summarization tasks. \tingyao{add more reference maybe?} \citet{zhang2021emailsum} proposed a hierarchical model based on HMNet \cite{zhu2020hierarchical} but for email summarization perform well. Similar to both works, we take HMNet hierarchical structure but use Longformer as backbone for our QA summarization task. We take advantage of both token-level and sentence-level representation learning in a hierarchical architecture. We think each QA pair can be treated as individual turn, so we apply the similar strategy as \cite{zhang2021emailsum} but different inputs to adapt our dataset. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{fig/multi-task-led.pdf}
    \caption{Architecture of \model.}
    \label{fig:dedupled}
    \vspace{-0.5cm}
\end{figure}

%https://docs.google.com/drawings/d/1wakF-WN4GDrh4VWyrI4fGuGXD9fVbitMJ49oHp3W7Ak/edit?usp=sharing



\paragraph{DedupLED} While pre-trained encoder-decoder models, including LED, are known to be powerful summarization solutions, they do not explicitly implement deduplication functionality. Inspired by BertSumExt, we consider incorporating a classifier layer optimized to extract the original seed QA pairs into an LED model and fine-tuning the LED model via multi-task learning, which we refer to as \model.
%
Figure~\ref{fig:dedupled} depicts the model architecture. The classifier layer is trained to select the original seed QA pairs, so the shared encoder learns to detect duplicate information while the decoder is optimized to generate a summary. 
%
In the training time, \model{} uses the original seed QA pair information in addition to the gold-standard summaries in the training data. We would like to note that \model{} does not require any additional information other than input QA pairs in the summary generation phase. %\yoshi{Rewrote the description. Can you check?}
%Finally, we consider a multi-task LED model, which we call DedupLED. As shown in Figure~\ref{fig:dedupled}, this model has two objectives: the main objective is to generate an abstractive summary of the input QAs and the auxiliary objective is to classify if an input QA is one of the seed QAs we selected in Sub-task 1 (Section~\ref{sec:annotation}). The goal of the auxiliary objective is to help the model to remove duplication from the input, thus we call it DedupLED. 
%\textbf{LED multi-task.} \xiaolan{}
%\yoshi{What about calling this DedupLED or something like that in a similar manner as Hierarchical LED?}
%\tingyao{show model architecture?}

==> EMNLP-2022 CoQASum/sections/problem.tex <==
Let $D$ denote a dataset of questions and answers on individual entities $\{e_{1}, e_{2},...,e_{\left|D \right|}\}$ (e.g., products or hotels).
%, e.g., a product or a hotel.
For every entity $e$, we define a set of question-answer pairs $QA_e=\{(q_i, a_i)\}^{|QA_e|}_{i=1}$, where the question $q_i$ and the answer $a_i$ are sequences of tokens $q_i = (w_1,...,w_n)$ and $a_i = (a_1, ..., a_m)$\footnote{Note that one question can have multiple answers, but we use this ``flat'' notation for simplicity. Thus, there can exist $q_i = q_j$ for some $i \ne j$. %\yoshi{Verbose. We should rephrase.}
}.
%
Given a set of QA pairs for an entity $e$, the \task{} task is 
%our goal aims
to generate a natural language summary $S_{e}$ from $QA_e$.

% \yoshi{The following paragraph may be unnecessary, especially if the figure is explained in the intro.}
% As shown in Figure~\ref{fig:example}, \task\ problem takes multiple questions and answers of a single entity, e.g., a puzzle board product, as the input (Figure~\ref{fig:example} (a)) and aims at producing a declarative summary that highlights all the key information \tingyao{do we need to highlight in the figure?} from the input (Figure~\ref{fig:example} (b)).

\begin{comment}

=> We will start with a small set of QA pairs.

\textbf{Challenges}

There are several key factors that distinguish Q\&A postings with reviews:
Incorporate both factual information \& subjective information. Unlike reviews, which often only contain subjective information (or opinions), Q\&A often contain both factual information and subjective information. We want our summary to include both.
The style of Q\&A. Instead of maintaining the original format, we want to summarize them in the declarative form. In other words, it is similar to “tell a story from hundreds of Q\&A pairs”. 

\textbf{Baselines}

Two steps: summarize questions and then summarize answers for the selected question.
Multi-document summarization: summarize multiple concatenated Q\&A pairs using existing multi-doc summarization methods.



\end{comment}










% Datasets
% Amazon Q&As.
% On shared GPU: /home/ubuntu/shared/amazon_qa
% 1,025,628 questions and 4,019,744 answers
% Indeed Q&A (internal)
% On shared GPU: /home/ubuntu/shared/indeed_qa
% 208,553 questions and 919,656 answers


==> EMNLP-2022 CoQASum/sections/related-work.tex <==
%\yoshi{Take 1. Feel free to edit/leave comments. Please be critical.}
%\yoshi{Will try to expand the related papers and dump the descriptions}
%\url{https://docs.google.com/document/d/1ZlfPZ17ee14oWmBUQXBVYemI2AUes4YciEVeySohBjY/edit#bookmark=id.tu155yrelnr3}
%\paragraph{Opinion Summarization}
Opinion summarization~\cite{OpinionSummarizationSIGIR2022Tutorial}
%\cite{suhara-etal-2020-opiniondigest} 
aims to create a summary from multiple customer reviews. While opinion summarization is relevant to \task{} as it summarizes consumer-generated text, customer reviews are significantly different from QA pairs in CQA as they are self-contained and tend to contain more subjective information. Recent opinion summarization models have adopted pre-trained LMs (LED) for summarizing multiple reviews~\cite{oved-levy-2021-pass,iso-etal-2022-comparative}. 

%\paragraph{Answer Summarization}
A line of work studies on summarizing answers in CQA, which can be categorized into extractive models~\cite{liu2008understanding,chan-etal-2012-community,Deng:2020:AAAI,Deng:2020:SIGIR} and abstractive models~\cite{AnswerSumm,chowdhury2021neural}.
%
Among them, \citet{CQASumm} created a benchmark by selecting the best answer as the reference summary, and \citet{AnswerSumm} has collected professionally written reference summaries for answer summarization.
%
Our \task{} differs from answer summarization as we consider multiple QAs as input, which offers unique challenges not in answer summarization.


%\paragraph{Dialog Summarization}
Another line of work in dialog summarization has created new benchmarks for E-mail threads~\cite{zhang2021emailsum}, customer support conversations~\cite{feigenblat-etal-2021-tweetsumm-dialog}, conversations in multiple domains~\cite{fabbri-etal-2021-convosumm}, and forum discussions~\cite{khalman-etal-2021-forumsum-multi}.
%
\task{} is similar to those tasks in creating abstractive summaries from multiple turn-taking conversations between more than one user. Meanwhile, we also found that \task\ tends to contain more duplication in the input by nature as the compression ratio (i.e., input length/summary length) of \corpus\ is $10.88\%$, which is smaller than EmailSum ($29.38\%$) and ForumSum ($11.85\%$).
%
We also tested HierLED, a variant of the strongest baseline for E-mail thread summarization, and confirmed that \model{} performs better than HierLED, indicating that \task{} offers unique challenges that are not in E-mail summarization.
%We also tested HierLED, which is known to be the strongest baseline for E-mail thread summarization, and have confirmed that \task{} contains more duplicate information by nature, which should be addressed to make a concise summary. 

%\yoshi{A survey paper on this topic \url{https://arxiv.org/abs/2107.03175} Will add ForumSum later} 

% \paragraph{Community-based Question Answering}
% \todo{Add papers about information extraction from CQA etc.}
% A line of work in CQA has been studied in NLP.


% \paragraph{Dialog Summarization}
% Another line of work in dialog summarization focuses on summarizing interactive conversations between multiple people. EmailSum 


% \begin{itemize}
%     \item EmailSum (ACL 21)~\cite{zhang-etal-2021-emailsum}
%     \item TweetSumm (EMNLP 21 Findings)~\cite{}
%     \item RepSum (ACL 21)~\cite{fu-etal-2021-repsum}
%     \item AnswerSumm~\cite{AnswerSumm}
% \end{itemize}

% Our work is similar to dialog summarization but different with respect to \todo{clarify the difference.}


==> sections/introduction_old.tex <==
\begin{figure}[t]
\includegraphics[width=0.49\textwidth]{fig/example.pdf}
    \caption{Example of the \task\ task.}
    \label{fig:amazon_qa}
\label{fig:example}
\end{figure}
% Figure link: https://docs.google.com/drawings/d/1MDoUwrOnHs-aU6p-Y6lmJlDcf9VzqbC1YM5yU-imcls/edit?usp=sharing

%Besides reviews, many e-service such as Amazon, Indeed, etc. websites now provide Questions and Answers (Q\&A) functionality for users to post their questions and also provide answers for others. (See the provided examples in \Cref{fig:indeed_qa}, \Cref{fig:amazon_qa}). Thus, Q\&A becomes an important resource for people to acquire the desired information. Meanwhile, the number of Q\&A pairs is consistently growing, which makes it hard for users to quickly digest information mentioned in existing Q\&As. Although most e-service consists of various items with question-answering data and reviews, we found there are some common properties between. (1) Most of product contains multiple questions and answers; (2) Many questions are repetitive and sometimes are either too short or too long that is unclear what the customers want to ask; (3) Answers are quite different from customers if it is an open questions because people tend to answer based on their experience or preference. Base on above properties, it becomes harder for the users to obtain useful and concrete information in just a couple of minutes. 

%\hl{

E-commerce platforms have became an essential component in our daily life. People nowadays use such platforms to perform a variety of tasks from online shopping, hotel/restaurant booking, to even job searching. Most of them use Community Question Answering (CQA) to help user acquire additional information about an entity (e.g., a product or a hotel). \kenneth{The paper didn't explain what is an ``entity''. You kinda need to clarify it, as in NLP an ``entity'' means something quite specific.}, such as the serving time of the breakfast in a hotel or the warranty of a product.\kenneth{I would use a different example. Since you want to emphasize ``extra'' information, I'd use some information that is obviously NOT in the manual.}
While such information can greatly benefit users in the decision making process, accessing the information mentioned in existing QAs is not always easy, especially when users do not know what to ask but still want to digest the important information the others mentioned.
This is because there often exits a large number of QAs with heavily repetitive questions and answers.
To address this issue, our goal is to summarize a collection of QAs from an entity (Figure~\ref{fig:example} (a)) into a concise and declaritive summary (Figure~\ref{fig:example} (b)), which we refer as the \textit{\task\ problem}.\kenneth{This is minor, BUT why not say it's ``CQA Summarization''? People know what CQA is.}

Unlike existing question and answering summarization works~\cite{see-etal-2017-get, liu2008understanding, deng2020joint}, which mainly focus on summarizing answers for one given question, the \task\ problem considers a collection of questions and their answers as the input.\kenneth{This is correct. So why did you decide to use the same name? ``QA Summarization'' has been used I think.}
Besides, the \task\ problem highlights two properties for a desired summary. First, like other summarization tasks, we want to exclude repetitive content by producing a \textit{concise} summary.
Second, instead of presenting a set of QAs, we want to generate a \textit{declarative} summary (i.e., summary in plain text) to further help readers quickly and easily digest the information.\kenneth{Now I see where does the word come from. BUT ``declarative'' is still quite confusing. I would use a more simple word.}
This property further makes existing opinion summarization solutions~\cite{meansum, suhara-etal-2020-opiniondigest}\todo{add more} unsuitable to solve the \task\ problem as they mainly takes plain text, i.e., reviews, as the input and rarely perform style transfer during the summarization process.

\kenneth{One argument missing here is why this is different from traditional summarization task. Because CQA data tends to be more repetitive?}

\kenneth{A higher-level argument (which may or may not be important) for CQA is that users with different needs can find what they want in the QAs. This paper kinda wants to say that users generally want to know the same set of information, which motivates the generation of summary. Not sure how important this is, but proably good to think about.}

A key challenge of the \task\ problem is the lack of training examples since none of the existing summarization benchmarks take a collection of questions and answers as the input and produce a declarative summary.
To address this challenge, we proposed a non-trivial data annotation process and created a benchmark dataset. With the benchmark dataset, we are then able to compare and study difference summarization models. Our contributions of the paper are as follows:
\begin{itemize}
    \item We propose a novel \task\ problem that takes multiple questions and answers from an entity as the input and generates a summary in the declarative form (i.e., plain text) (Section~\ref{sec:problem}). 
    \item We present a non-trivial data annotation framework to collect reference summaries and build the first benchmark dataset, which includes annotated summaries for $1440$ entities with $11.5K$ QA pairs, on Amazon CQA corpus~\cite{wan2016modeling}. Our annotation framework can also be applied for CQA corpus in other domains (Section~\ref{sec:corpus}). 
    \item We conduct a comprehensive empirical experiments for a series of extractive and abstractive summarization models and evaluated these models with both automatic and human evaluation. Through our experiments, we further establish strong baselines for the \task\ problem (Section~\ref{sec:models} and Section~\ref{sec:evaluation}). 
\end{itemize}

\kenneth{I don't think you need to have this outline for the paper for NLP papers. Can cut when need more space.}


%\todo{write a paragraph summarizing the key content and contribution of the paper.}\tingyao{I am done, feel free to modify this section}
\xiaolan{made a pass.}



%\begin{figure*}
%    \includegraphics[width=0.4\textwidth]{fig/indeed_qa.png}
%    \caption{Question \& Answering pairs for Dairy Queen at Indeed.com.}
%    \label{fig:indeed_qa}
%\end{figure*}

%\begin{figure*}
%    \includegraphics[width=0.4\textwidth]{fig/amazon_qa.png}
%    \caption{Question \& Answering pairs for "Conair HLM10 Hot Lather Machine" at Amazon.com.}
%    \label{fig:amazon_qa}
%\end{figure*}



%Existing summarization efforts on question and answering is mostly over a single question, i.e., how to summarize answers for a given question. \cite{see-etal-2017-get, liu2008understanding, deng2020joint} \todo{add for deng}. However, little work has been done over for summarizing all Q\&A postings for a given entity. \citet{suhara-etal-2020-opiniondigest} summarizes hundreds of user reviews, providing summaries for Q\&As is particularly helpful for users who want to digest information in Q\&A sessions but do not want to spend too much time browsing them, we take this advantage of our Q\&As summary. In addition, to make the summary concise, instead of presenting a set of selected Q\&As, we also want to summarize them in the declarative form, i.e., plain text. Thus, the core question we want to solve in this project is “how to summarize the most important, or most frequently asked questions in the Q\&A sessions?”. 
\iffalse

We introduce the QA summarization task as a result of the preceding intuition and existing limitation. Given a set of questions and answers, generate a declarative and informative summary. As far as we know, we are the first to propose the task. Our benchmark is built upon Amazon QA dataset, one of diverse and large-scale CQA dataset collected by \cite{wan2016modeling} from the product website. 
% xiaolan: I think we don't need to describe amazon QA dataset too much in the intro. Only highlight our dataset is enough. 
We first determined which items had lower quality QAs and obtained 1440 items and 11520 QA pairs in total. We then use human annotation in two steps to collect high-quality summaries. Finally, we use our dataset to establish strong baselines in three common summarization task approaches. 
% xiaolan: three common summarization approaches is not very clear. People may wonder "what three common approaches?" 
In general, we believe our proposed framework can be applied to any CQAs other than Amazon QA.
% xiaolan: sequence of the description is a bit twisted. I guess the framework here is about the annotation. So, in this paragraph, you first talked about problem -> annotation -> baselines -> annotation. Annotation appears twice. I believe it is better only mention it once.  



Overall, we claim the following contributions for our work.
\begin{itemize}
    \item We propose a new Amazon QA dataset as a high-quality resource for the QA summarization task.
    \item We conduct a thorough empirical model study and human evaluation analysis, which is critical for future research.
    \item Our framework is applicable not only to Amazon QA, but also to other domains of CQA dataset. 
\end{itemize}

Section \ref{sec:problem} defines our problem. Section \ref{sec:corpus} describes our framework for collecting the dataset. In Section \ref{sec:models}, we set up a comprehensive expriment and present both human and automatic evaluation in Section \ref{sec:evaluation}. In Section \ref{sec:analysis}, we conduct three different comparisons to analyze the experimental results.
\fi
